Hardware-Aware Static Optimization of Hyperdimensional Computations

Binary spatter code (BSC)-based hyperdimensional computing (HDC) is a highly error-resilient approximate computational paradigm suited for error-prone, emerging hardware platforms. In BSC HDC, the basic datatype is a hypervector, a typically large binary vector, where the size of the hypervector has a significant impact on the fidelity and resource usage of the computation. Typically, the hypervector size is dynamically tuned to deliver the desired accuracy; this process is time-consuming and often produces hypervector sizes that lack accuracy guarantees and produce poor results when reused for very similar workloads. We present Heim, a hardware-aware static analysis and optimization framework for BSC HD computations. Heim analytically derives the minimum hypervector size that minimizes resource usage and meets the target accuracy requirement. Heim guarantees the optimized computation converges to the user-provided accuracy target on expectation, even in the presence of hardware error. Heim deploys a novel static analysis procedure that unifies theoretical results from the neuroscience community to systematically optimize HD computations. We evaluate Heim against dynamic tuning-based optimization on 25 benchmark data structures. Given a 99% accuracy requirement, Heim-optimized computations achieve a 99.2%-100.0% median accuracy, up to 49.5% higher than dynamic tuning-based optimization, while achieving 1.15x-7.14x reductions in hypervector size compared to HD computations that achieve comparable query accuracy and finding parametrizations 30.0x-100167.4x faster than dynamic tuning-based approaches. We also use Heim to systematically evaluate the performance benefits of using analog CAMs and multiple-bit-per-cell ReRAM over conventional hardware, while maintaining iso-accuracy -- for both emerging technologies, we find usages where the emerging hardware imparts significant benefits.

==> background-scratch.tex <==
\begin{table}
\small
%\setlength{\tabcolsep}{2pt}
\begin{tabular}{|l|ll|ll|}
 \hline
\textbf{Operator} &\textbf{Notation} & \textbf{Intuitive Operation} & \textbf{Description} & 
 \textbf{Implementation}\\
 \hline
distance & $\distance{hv}{hv'}$ & $hv \subseteq hv'$ & distance between $hv$, $hv'$ & Hamming distance\\
binding & $hv \hdtimes hv'$ & $\tuple{hv,hv'}$ & bind $hv$, $hv'$ & bitwise exclusive-or\\
bundling & $hv + hv'$ & $\set{hv,hv'}$ & bundle $hv$, $hv'$ & bitwise majority\\
permute & $\hdperm{hv}{i}$ & - & permute $hv$ \codein{i} times & circular bit shift\\
random vector& - & - & generate a random code & random bit generation\\
\hline
\end{tabular}
\caption{BSC computation operations. Hypervectors are of size $\hvsize$.}
\label{fig:hdops}
\end{table}


==> big_exp_table.tex <==
\begin{figure}
\footnotesize
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{|c|c|cccccc|cccccc|c|cccccc|}
\hline
 Baseline & \multicolumn{7}{c|}{\textbf{\tool{}}}  & \multicolumn{6}{c|}{\textbf{Static} (\textit{dim=10000})} & \multicolumn{7}{c|}{\textbf{DT}}\\
 \hline
 &  & \multicolumn{6}{c|}{\textbf{accuracy}} & \multicolumn{6}{c|}{\textbf{accuracy}} &  & \multicolumn{6}{c|}{\textbf{accuracy}}\\
\textbf{benchmark}&\textit{dim}&\textit{med}&\textit{iqr}&\textit{min}&\textit{max}&\textit{std}&\textit{rat}&\textit{med}&\textit{iqr}&\textit{min}&\textit{max}&\textit{std}&\textit{rat}&\textit{dim}&\textit{med}&\textit{iqr}&\textit{min}&\textit{max}&\textit{std}&\textit{rat}\\
\hline

\textbf{set-100} & \textit{3407} & 99.5 & 0.5 & 98.0 & 100.0 & 0.5 & 92.0 & 98.0 & 2.1 & 93.5 & 100.0 & 1.5 & 25.0 & \textit{2016} & 97.5 & 3.0 & 88.5 & 100.0 & 2.3 & 16.0 \\
\textbf{set-200} & \textit{6807} & 100.0 & 0.5 & 98.5 & 100.0 & 0.5 & 93.0 & 98.0 & 2.0 & 94.0 & 100.0 & 1.2 & 22.0 & \textit{3865} & 97.0 & 2.0 & 91.0 & 100.0 & 1.7 & 16.0 \\
\textbf{set-300} & \textit{10208} & 99.8 & 1.0 & 97.0 & 100.0 & 0.6 & 87.0 & 99.0 & 1.5 & 97.5 & 100.0 & 0.8 & 73.0 & \textit{8049} & 99.0 & 1.0 & 97.0 & 100.0 & 0.8 & 66.0 \\
\textbf{set-400} & \textit{13608} & 99.5 & 0.6 & 97.5 & 100.0 & 0.6 & 86.0 & 98.5 & 1.5 & 95.0 & 100.0 & 1.1 & 31.0 & \textit{8324} & 98.0 & 1.0 & 94.0 & 100.0 & 1.0 & 17.0 \\
\textbf{set-500} & \textit{17009} & 99.5 & 1.0 & 98.0 & 100.0 & 0.5 & 88.0 & 98.0 & 1.5 & 94.0 & 100.0 & 1.3 & 21.0 & \textit{9394} & 97.2 & 3.0 & 92.0 & 100.0 & 2.0 & 15.0 \\
\hline
\textbf{kg-100} & \textit{3407} & 99.2 & 0.3 & 98.2 & 99.8 & 0.2 & 80.0 & 99.6 & 0.2 & 99.1 & 99.8 & 0.2 & 100.0 & \textit{3909} & 99.5 & 0.3 & 98.5 & 99.8 & 0.2 & 99.0 \\
\textbf{kg-200} & \textit{6807} & 99.3 & 0.3 & 98.8 & 99.6 & 0.2 & 89.0 & 98.0 & 0.5 & 96.8 & 98.7 & 0.4 & 0.0 & \textit{4908} & 98.1 & 0.4 & 97.0 & 98.8 & 0.4 & 0.0 \\
\textbf{kg-300} & \textit{10208} & 99.3 & 0.3 & 98.6 & 99.6 & 0.2 & 89.0 & 98.7 & 0.4 & 98.0 & 99.6 & 0.3 & 15.0 & \textit{8496} & 98.7 & 0.4 & 97.5 & 99.2 & 0.3 & 12.0 \\
\textbf{kg-400} & \textit{13608} & 99.3 & 0.3 & 98.7 & 99.8 & 0.2 & 90.0 & 98.7 & 0.4 & 97.7 & 99.5 & 0.3 & 17.0 & \textit{11254} & 98.6 & 0.4 & 97.9 & 99.3 & 0.3 & 13.0 \\
\textbf{kg-500} & \textit{17009} & 99.3 & 0.3 & 98.8 & 99.8 & 0.2 & 93.0 & 98.5 & 0.5 & 97.3 & 99.2 & 0.3 & 6.0 & \textit{13195} & 98.3 & 0.4 & 97.5 & 99.0 & 0.3 & 1.0 \\
\hline
\textbf{wta-a-4-100} & \textit{1509} & 100.0 & 0.5 & 99.0 & 100.0 & 0.3 & 99.0 & 94.5 & 3.5 & 88.5 & 100.0 & 2.7 & 4.0 & \textit{681} & 95.0 & 3.5 & 89.0 & 100.0 & 2.6 & 6.0 \\
\textbf{wta-a-8-200} & \textit{6119} & 100.0 & 0.0 & 99.0 & 100.0 & 0.2 & 99.0 & 97.0 & 2.5 & 92.5 & 99.5 & 1.7 & 7.0 & \textit{3125} & 97.0 & 2.0 & 92.5 & 99.5 & 1.7 & 9.0 \\
\textbf{wta-a-12-300} & \textit{14157} & 100.0 & 0.0 & 99.5 & 100.0 & 0.2 & 100.0 & 99.0 & 1.0 & 96.0 & 100.0 & 0.9 & 61.0 & \textit{9318} & 99.0 & 1.0 & 96.0 & 100.0 & 0.9 & 68.0 \\
\textbf{wta-a-16-400} & \textit{25804} & 100.0 & 0.0 & 99.5 & 100.0 & 0.1 & 100.0 & 98.5 & 1.1 & 96.0 & 100.0 & 0.9 & 35.0 & \textit{15897} & 98.5 & 1.0 & 96.0 & 100.0 & 0.9 & 37.0 \\
\textbf{wta-a-20-500} & \textit{41186} & 100.0 & 0.0 & 99.5 & 100.0 & 0.1 & 100.0 & 99.0 & 1.0 & 95.5 & 100.0 & 0.8 & 66.0 & \textit{27241} & 99.0 & 1.0 & 95.5 & 100.0 & 0.8 & 70.0 \\
\hline
\textbf{match-10-2} & \textit{1376} & 99.8 & 0.2 & 99.4 & 100.0 & 0.1 & 100.0 & 100.0 & 0.1 & 99.7 & 100.0 & 0.1 & 100.0 & \textit{1604} & 98.4 & 1.3 & 95.5 & 99.8 & 0.9 & 22.0 \\
\textbf{match-20-4} & \textit{4224} & 99.9 & 0.2 & 99.4 & 100.0 & 0.1 & 100.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 97.4 & 2.0 & 92.6 & 100.0 & 1.6 & 14.0 \\
\textbf{match-30-6} & \textit{8633} & 99.6 & 0.3 & 99.0 & 100.0 & 0.2 & 100.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 96.3 & 2.9 & 88.2 & 100.0 & 2.2 & 10.0 \\
\textbf{match-40-8} & \textit{14601} & 99.7 & 0.3 & 99.0 & 100.0 & 0.2 & 98.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 95.1 & 2.4 & 90.4 & 100.0 & 2.1 & 4.0 \\
\textbf{match-50-10} & \textit{22129} & 99.8 & 0.3 & 99.3 & 100.0 & 0.2 & 100.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 94.1 & 3.7 & 89.1 & 99.2 & 2.5 & 2.0 \\
\hline
\textbf{nfa-6} & \textit{3594} & 100.0 & 0.0 & 98.0 & 100.0 & 0.3 & 98.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 82.0 & 8.1 & 64.0 & 98.0 & 6.5 & 0.0 \\
\textbf{nfa-8} & \textit{6517} & 100.0 & 0.0 & 98.5 & 100.0 & 0.3 & 99.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 71.5 & 10.1 & 50.5 & 89.0 & 8.4 & 0.0 \\
\textbf{nfa-10} & \textit{10387} & 100.0 & 0.0 & 98.5 & 100.0 & 0.3 & 99.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 66.5 & 13.6 & 42.5 & 90.5 & 9.0 & 0.0 \\
\textbf{nfa-12} & \textit{15235} & 100.0 & 0.0 & 98.5 & 100.0 & 0.2 & 99.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 60.7 & 8.1 & 45.0 & 73.5 & 6.0 & 0.0 \\
\textbf{nfa-14} & \textit{21088} & 100.0 & 0.0 & 99.0 & 100.0 & 0.2 & 100.0 & 100.0 & 0.0 & 100.0 & 100.0 & 0.0 & 100.0 & \textit{100000} & 54.5 & 8.6 & 37.0 & 71.0 & 7.0 & 0.0 \\
\hline


\hline
\end{tabular}
\caption{Derived hypervector dimensions and empirical accuracy measures for 100 random data structures. \codein{a} is short for \codein{analogy}, \codein{kg} is short for \codein{knowledge-graph}. The numbers in benchmark names indicate the parameters (sizes) of the benchmarks as previously described (e.g., number of codes in set). Target accuracy is \codein{99.0}\%. All accuracy measures are shown 100$\times$ the original number.}
\label{table:empirical:accuracy}
\end{figure}

==> datastructures.tex <==
% moved to supplementary materials

==> figures/sources.tex <==


// overview figure

https://docs.google.com/drawings/d/1ckrjo_dsgqZ__f3bm0-WyK7_E0sQqQBfUFjnc3DyeP0/edit?usp=sharing

// distribution figure

https://docs.google.com/drawings/d/171s47rJMwQUcKoIDBTy_J060WjMZ5ITX_wpbZoQ1YNU/edit?usp=sharing

// static part overview figure
https://docs.google.com/drawings/d/1ckrjo_dsgqZ__f3bm0-WyK7_E0sQqQBfUFjnc3DyeP0/edit

// dynamic part overview figure
https://docs.google.com/drawings/d/1tLup_JudG3ZyUKbz4nPdyc1RgUUovesm7j4L4HOJCKc/edit

==> language-example.tex <==
\subsection{Illustrative Example: Knowledge Graph}\label{sec:datastructure:knowledgegraph}


\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{lllp{5cm}}
\textbf{Knowledge Graph / API call} & \textbf{type} & \textbf{description} & \textbf{\tool{} specification fragment}\\ \hline
\texttt{\lit{KG}(VarExpr,VarExpr',VarExpr'',N)} & ctor & instantiation & \syn{edge} = \lit{prod}(VarExpr,VarExpr',VarExpr'')\\
& & & \syn{ds} = \lit{sum}(N,\syn{edge})\\
\texttt{\lit{addVertex}(edges)} & modify & add vertex & \\
\texttt{\lit{hasEdge}(edge,acc,fp,fn)} & query & has edge & \lit{thr-query}(\syn{edge},\syn{ds},1,acc,fp,fn)\\\hline
\end{tabular}
\vspace{5pt}
\caption{Knowledge graph API and \tool{} specification fragments. The \texttt{VarExpr}, \texttt{VarExpr'}, and \texttt{VarExpr''} are \tool{} concept, relation, and interaction abstract HD variables expressions from the grammar in Figure~\ref{fig:grammar:speclang}. \texttt{N} is the degree of the graph. The \texttt{acc}, \texttt{fp}, \texttt{fn} rates are the accuracy, false positive, and false negative rates for the query respectively.}
\label{table:ds:knowledge}
\end{table}

We present a novel HD analysis-amenable knowledge graph representation that maintains per-node edge lists in item memory. A knowledge graph is a directed, labelled graph. Edges are labeled with codes from the relations codebook \codein{VarExpr'} and nodes are uniquely identified by codes from the concept codebook \codein{VarExpr}. The direction of each edge is indicated by an interaction code (\codein{VarExpr''}). Figure~\ref{table:ds:knowledge} presents the knowledge graph API and the \tool{} specification fragment associated with each API endpoint. The API supports creating knowledge graphs, adding nodes and edges to knowledge graphs, and filtering the nodes in the knowledge graph by an edge:

\begin{itemize}[leftmargin=*]
\item{}\textbf{Constructor (\texttt{\lit{KG}}).} The constructor specifies the maximum degree of the graph.
\item{}\textbf{Adding Vertices and Edges (\texttt{\lit{addVertex}}).} This API adds a vertex with its incident edge list to the graph.
\item{}\textbf{Querying Edges (\texttt{\lit{hasEdge}}).} This API specifies an edge query with accuracy requirements.
\end{itemize}


==> old-texfiles/tech-analysis-backup.tex <==
\section{\tool{} Accuracy Analysis}\label{sec:accuracy:analysis}

\tool{}'s static optimizer (Section~\ref{sec:optimizer}) leverages a static accuracy analysis procedure that computes the accuracy given the hypervector size $\hvsize$ (and finds the optimal distance threshold for thresholding queries) for the data structure query encoded in the accuracy constraint.
%Because the accuracy analysis makes use of multiple analytical models that make different independence assumptions, this analysis additionally returns an \textit{independence constraint} that must hold for the analysis to be valid.
%Section~\ref{sec:mutual:independence} introduces the independence constraints.
Section~\ref{sec:model:intuition} presents the intuition of the analytical model, which is rigorously presented in Section~\ref{sec:analyticalmodel}.
Section~\ref{sec:thr:analysis} presents the accuracy analysis procedure for thresholding queries (\codein{thrAccAnalysis}), and Section~\ref{sec:wta:analysis} presents the accuracy analysis procedure for WTA queries (\codein{wtaAccAnalysis}).

\subsection{Analytical Model Intuition}\label{sec:model:intuition}

\begin{figure}
\includegraphics[width=0.9\linewidth]{figures/Distribution.pdf}
\caption{Visualization of distribution-based accuracy analysis. For thresholding queries, the query accuracy is \swatch{blue} + \swatch{lightred}, false positive rate is \swatch{hotpink}, false negative probability is \swatch{violet}. \luke{better change y-axis label to to probability density}}
\label{fig:distr}
\end{figure}

Figure~\ref{fig:distr} visually depicts the analytical models that we derive in our analysis, which are rigorously derived in Section~\ref{sec:analyticalmodel}. Given a data structure query $|q \cap ds|\ge k$ with hypervector size $\hvsize$ and a hardware error probability $p$, we analytically derive the in-set ($|q \cap ds|\ge k$) and not-in-set ($|q \cap ds|< k$) distance distributions with the analytical models. The in-set and not-in-set probability distributions capture the distribution of distances between the query and data structure hypervectors $\distance{q}{ds}$ when $|q \cap ds|\ge k$ and $|q \cap ds|< k$ respectively.

Intuitively, the in-set distribution captures the probability that at least $k$ elements in the query are contained within the data structure, and the not-in-set distribution captures the probability that less than $k$ in the query are contained with by the data structure. Both in-set and not-in-set distances follow probability distributions  rather than resolve to a concrete value.. The query-data structure distance is non-deterministic because the codebook $\codebook$ is randomly generated, and the hardware non-deterministically introduces error.

\noindent\textbf{Deriving the $\Phi_S$,$\Phi_{NS}$ Distributions.} We use the analytical model presented in Section~\ref{sec:analyticalmodel} to derive the in-set and not-in-set ($\Phi_S$, $\Phi_{NS}$) distance distributions. The analytical model $\analyticalmodel(q,ds,k,n,hw) \rightarrow \tuple{indepCstr,\Phi_{S},\Phi_{NS}}$ takes as input the query and data structure to analyze ($q$ and $ds$), the query parameter $k$, the hypervector size $n$, the hardware model $hw$, and returns the in-set and not-in-set ($\Phi_S$, $\Phi_{NS}$) distributions and the mutual independence constraint that must hold for the analysis to be valid.

\subsection{Accuracy Analysis for Thresholding Queries}\label{sec:thr:analysis} 

For thresholding queries, the \textit{accuracy} of the query is determined by computing the area covered by the non-overlapping portions of the in-set and not-in-set distributions. The \textit{distance threshold} $\threshold$ partitions the distribution of distances into 'in-set' and 'not-in-set' regions. The overlapping area to the left of the distance threshold is the false positive rate, and the overlapping region to the right of the distance threshold is the false negative rate. The \textit{threshold optimization algorithm} uses these analytical distributions to compute the true positive and true negative rates of different thresholds.
 
 
%\luke{So the notions like ``in-set'', ``not-in-set'' do not represent the subset case well; and ``$m$'', ``data structure size'' do not represent the type-III QDS well, where $\mu$ and $\sigma$ depend on the sizes of the ds multiplicant sets. Should we just say that this section is an illustrative example that uses type-I QDS?}
%\sara{definitely not.}

 \begin{figure}[t]
\begin{minipage}{\linewidth}
\small
\begin{algorithmic}[1]
\Procedure{getThreshold}{$\Phi_S,\Phi_{NS}$,reqAcc,reqFp,reqFn}
\State $\threshold_l$ = $CDF(\Phi_{S})^{-1}(1-reqFn)$
\State $\threshold_h$ = $CDF(\Phi_{NS})^{-1}(reqFp)$
\If{$\threshold_l > \threshold_h$}
    \State \textbf{return} $\tuple{-1,False}$
\EndIf
%\State $succ$ = True
\State $x$ = \lit{getIntersection}($PDF(\Phi_S),PDF(\Phi_{NS})$)
\If{$\threshold_h \le x$}
    \State $\threshold$ = $\threshold_h$
\ElsIf{$\threshold_l \ge x$}
    \State $\threshold$ = $\threshold_l$
\Else
    \State $\threshold$ = $x$
\EndIf
\State $acc$ = $1-\frac12(CDF(\Phi_{NS})(\threshold)+1-CDF(\Phi_{S})(\threshold))$
\State $succ$ = $acc\ge reqAcc$
\State \textbf{return} $\tuple{\threshold,succ}$
\EndProcedure
\Procedure{thrAccAnalysis}{hw,q,ds,n,k,reqAcc,reqFp,reqFn}
%\State \textbf{float} p = \lit{getBitFlipProb}(hw)
\State $\tuple{indepCstr,\Phi_S,\Phi_{NS}}$ = $\analyticalmodel(q,ds,k,n,hw)$
\State $\tuple{\threshold,succ}$ = \lit{getThreshold}($\Phi_S,\Phi_{NS}$,reqAcc,reqFp,reqFn)
\State \textbf{return} $\tuple{succ,indepCstr,\threshold}$
\EndProcedure
\end{algorithmic}
\caption{\tool{} \algname{getThreshold} and \algname{thrAccAnalysis} algorithms}
\label{algo:get:accuracy}
\end{minipage}
\end{figure}

\subsubsection{\mycodeheading{Threshold Optimization}{getThreshold}}

\tool{} finds the optimal distance threshold $\threshold$ for the given in-set ($\Phi_S$) and not-in-set distributions ($\Phi_{NS}$) and a set of upper bounds on false negative and false positive probabilities ($reqFn$ and $reqFp$).
The algorithm pseudo code is shown in Figure~\ref{algo:get:accuracy}.
Given a candidate threshold $\threshold$, $fn=1-CDF(\Phi_{S})(\threshold)$ is the false negative probability, and $fp=CDF(\Phi_{NS})(\threshold)$ is the false positive probability for that threshold.
With the increase of $\threshold$, $fn$ decreases and $fp$ increases.
Therefore, the false positive requirement $recFp$ sets an upper bound $\threshold_h$ and the false negative requirement $recFn$ sets a lower bound $\threshold_l$ for the threshold $\threshold$.
If $\threshold_l > \threshold_h$, there is no $\threshold$ satisfying both $recFn$ and $recFp$ requirements.
Otherwise, any $\threshold\in [\threshold_l,\threshold_h]$ satisfies both constraints, and we aim to choose one $\threshold$ that maximizes the accuracy $1-\frac{fp+fn}2$ (assuming balanced positive and negative queries).
Denote $x$ as the middle intersection of two distributions, i.e., $PDF(\Phi_S)(x)=PDF(\Phi_{NS})(x),\mu_S<x<\mu_{NS}$.
Solving $x$ is trivial as $PDF(\Phi_S)(x)=PDF(\Phi_{NS})(x)$ is a quadratic function of $x$.
Note that in the middle region, $(fp+fn)$ decreases monotonically when $\threshold<x$, and increases monotonically when $\threshold>x$.
Therefore, \tool{} lets $\threshold=\threshold_h$ when $\threshold_h\le x$, $\threshold=\threshold_l$ when $\threshold_l\ge x$, and $\threshold=x$ when $\threshold_l\le x\le \threshold_h$.

\subsubsection{\mycodeheading{Accuracy Analysis Algorithm}{thrAccAnalysis}}\label{sec:thrAccAnalysis}
The accuracy analysis (\algname{thrAccAnalysis}) algorithm solves for the optimal threshold and lower accuracy bound for the query described in the accuracy constraint.
The algorithm pseudo code is shown in Figure~\ref{algo:get:accuracy}.
The \codein{thrAccAnalysis} function accepts as input a query and data structure, a hypervector size (\codein{n}), the minimum number of query elements contained within the data structure (\codein{k}), the hardware error model (\codein{hw}), an accuracy lower bound (\codein{reqAcc}) and a false positive rate/false negative rate upper bound (\codein{reqFp}, \codein{reqFn}). The accuracy analysis translates the hardware error model to a single bit flip error probability upper bound $p$ (Section~\ref{sec:inferbfp}) and then invokes the analytical model $\analyticalmodel(q,ds,k,n,hw)$ (Section~\ref{sec:analyticalmodel}) on the query and data structure HD expressions ($q$ and $ds$), the hypervector size ($n$), the hardware error probability $p$, and the number of query elements $k$ to derive the in-set and not-in-set distributions $\Phi_S,\Phi_{NS}$ and the mutual independence constraint $indepCstr$. 

 
 The algorithm then computes the optimal distance threshold $\threshold$ from distributions $\Phi_S,\Phi_{NS}$ that delivers false positive and false negative rate less than the false-positive/false negative upper bounds ($fp \leq reqFp$ and $fn \leq reqFn$) and maximizes the accuracy. If such a threshold cannot be found, the algorithm sets \codein{succ=\syn{false}}. Provided a threshold is successfully found ($succ=fp \leq reqFp \wedge fn \leq reqFn \wedge 1-\frac{fp + fn}2 \geq reqAcc$), the algorithm then returns the optimal threshold, the mutual independence constraint that must hold, and whether this parametrization satisfies the provided accuracy constraint ($\tuple{succ,indepCstr,\threshold}$).

\subsection{Accuracy Analysis for WTA Queries}\label{sec:wta:analysis}

 \begin{figure}[t]
 \small
\begin{minipage}{\linewidth}
%\small
\begin{algorithmic}[1]
\Procedure{wtaAccAnalysis}{hw,q,ds,n,k,w,m,x,t,x'}
%\State \textbf{float} p = \lit{getBitFlipProb}(hw)
\State $\tuple{indepCstr,\Phi_S,\Phi_{NS}}$ = $\analyticalmodel(q,ds,k,n,hw)$
\State $\tuple{acc,prob}$ = \lit{computeAccuracies}($\Phi_S,\Phi_{NS}$,w,m,t)
\State $succ$ = $acc\ge x\wedge prob\ge x'$
\State \textbf{return} $\tuple{succ,indepCstr}$
\EndProcedure
\end{algorithmic}
\caption{\tool{} \algname{wtaAccAnalysis} algorithms}
\label{algo:wta:accuracy}
\end{minipage}
\end{figure}

The accuracy analysis procedure for WTA queries (\codein{wtaAccAnalysis}) also uses the analytical model $M$ to get the in-set and not-in-set distributions ($\Phi_S$ and $\Phi_{NS}$).
%The inputs of a WTA query are the number of winners $w$, a data structure vector $ds$ and a codebook of $m$ vectors, when it is known that $w$ vectors in $m$ are positives ($\distance{q}{ds}\sim \Phi_S$) and the other $m-w$ are negatives ($\distance{q}{ds}\sim \Phi_{NS}$).
The WTA queries assume that $w$ vectors in $m$ are positives ($\distance{q}{ds}\sim \Phi_S$) and the other $m-w$ are negatives ($\distance{q}{ds}\sim \Phi_{NS}$).
The WTA query simply returns the $w$ vectors that have the smallest distance to the data structure vector among the $m$ vectors in codebook.

\subsubsection{\mycodeheading{Accuracy Analysis Algorithm}{wtaAccAnalysis}}
Figure~\ref{algo:wta:accuracy} presents the pseudo code for WTA accuracy analysis.
Similarly as \codein{thrAccAnalysis}, it first gets $\Phi_S$ and $\Phi_{NS}$ from the analytical model (Section~\ref{sec:analyticalmodel}), then computes the expected accuracies $acc$ and $prob$ (Section~\ref{sec:wta:acc:compute}), for the two accuracy constraints respectively.
The accuracy $acc$ of the WTA query is the probability that the returned $w$ vectors are exactly the $w$ positives.
The first accuracy constraint requires $acc\ge x$.
The second accuracy constraint defines $prob$ as the probability that the $w$ positives are all among the top-$t$ in the codebook with the smallest distances to the data structure $ds$, and requires that $prob\ge x'$.
The analysis is successful iff the two constraints are both satisfied.
Finally the algorithm returns whether the analysis is successful, and the independent constraints.

\subsubsection{\mycodeheading{Accuracies Computation}{computeAccuracies}}\label{sec:wta:acc:compute}

We present how $acc$ and $prob$ are computed in this section.
We start with $acc$.
We denote the WTA query accuracy as $acc(w,m,\Phi_S,\Phi_{NS})$.

Frady et al.~\cite{frady2018theory} developed a perception theory that gives the expected WTA accuracy when $w=1$ as follows
\begin{equation}\label{eq:frady:wta:1}
    acc(1,m,\Phi_S,\Phi_{NS}) = \int_{-\infty}^{\infty}PDF(\Phi_S)(x)(1-CDF(\Phi_{NS})(x))^{m-1}dx
\end{equation}
An intuitive explanation of the above equation is that when the one positive vector has distance $x$ to $ds$ (with probability density $PDF(\Phi_S)(x)$), the result is accurate iff the other $m-1$ distractor vectors all have a distance greater than $x$ (each independently with probability $1-CDF(\Phi_{NS})(x)$), and the result is the integral of it for all possible $x$.

\noindent\textbf{More Than One Winner}
We extend the theory to handle the general cases when $w>1$.
Following the intuition of (\ref{eq:frady:wta:1}), if we have the probability density function of the maximum of distances of $w$ positive vectors $PDF(MAX_{w,\Phi_S})$, then
\[
acc(w,m,\Phi_S,\Phi_{NS}) = \int_{-\infty}^{\infty}PDF(MAX_{w,\Phi_S})(x)(1-CDF(\Phi_{NS})(x))^{m-w}dx
\]
because the results are accurate (i.e., the returned $w$ vectors are all positives) iff the maximum distance of the $w$ positives is no greater than the minimum of the $m-w$ negatives.

We then derive $PDF(MAX_{w,\Phi_S})$.
First, we have 
\[
CDF(MAX_{w,\Phi_S})(x) = CDF(\Phi_S)^w(x)
\]
because $MAX_{w,\Phi_S}\le x$ iff all $w$ positive distances are no greater than $x$, each independently with probability $CDF(\Phi_S)(x)$. Then, with the relation of $CDF$ and $PDF$ and the chain rule, we have
\begin{equation}\label{eq:wta:pdf:max}
    PDF(MAX_{w,\Phi_S})(x) = CDF(MAX_{w,\Phi_S})'(x) = (CDF(\Phi_S)^w(x))' = wCDF(\Phi_S)^{w-1}(x)\cdot PDF(\Phi_S)(x)
\end{equation}
With (\ref{eq:wta:pdf:max}), we now conclude that
\begin{equation}\label{eq:wta:k}
    acc(w,m,\Phi_S,\Phi_{NS}) = \int_{-\infty}^{\infty}wCDF(\Phi_S)^{w-1}(x)PDF(\Phi_S)(x)(1-CDF(\Phi_{NS})(x))^{m-w}dx
\end{equation}

\noindent\textbf{Semi-Accuracy Constraint}
Besides specifying the desired accuracy, \tool{} also enables users to specify \emph{semi-accuracy constraint} for WTA queries, with the following form: with probability $x'$ the distances of the $w$ positives are all in the top-$t$ smallest.
In other words, there can be at most $t-w$ in the other $m-w$ vectors in the codebook that have a distance smaller than any positive, with probability $x'$.
To formulate this new constraint, we denote $prob(w,m,t,\Phi_S,\Phi_{NS})$ as the probability that $w$ positives all have at least top-$t$ smallest distances.

To calculate $prob(w,m,t,\Phi_S,\Phi_{NS})$, we enumerate the number of negatives that have a smaller distance than any positives ($i$), which should be no more than $t-w$.
For each $i$, and $MAX_{w,\Phi_S}=x$, the probability is that exactly $i$ negatives have smaller distances than $x$, each independently with probability $CDF(\Phi_{NS})(x)$, and the other $m-w-i$ negatives have greater distances than $x$, each independently with probability $1-CDF(\Phi_{NS})(x)$.
Therefore, we have
\[
\begin{array}{rl}
    &prob(w,m,t,\Phi_S,\Phi_{NS})=\\ &\sum_{i=0}^{t-w}\binom{m-w}{i}\cdot\int_{-\infty}^{\infty}PDF(MAX_{w,\Phi_S})CDF(\Phi_{NS})^{i}(x)(1-CDF(\Phi_{NS})(x))^{m-w-i}dx
\end{array}
\]

Substituting $PDF(MAX_{w,\Phi_S})$ with (\ref{eq:wta:pdf:max}), we have
\begin{equation}\label{eq:wta:prob}
\small
\begin{array}{rl}
    &prob(w,m,t,\Phi_S,\Phi_{NS})=\\ &\sum_{i=0}^{t-w}\binom{m-w}{i}\cdot\int_{-\infty}^{\infty}wCDF(\Phi_S)^{w-1}(x)PDF(\Phi_S)(x)CDF(\Phi_{NS})^{i}(x)(1-CDF(\Phi_{NS})(x))^{m-w-i}dx
\end{array}
\end{equation}

==> old-texfiles/tech-analysis.tex <==
\section{\tool{} Accuracy Analysis}\label{sec:accuracy:analysis}

\tool{}'s static optimizer (Section~\ref{sec:optimizer}) leverages a static accuracy analysis procedure that computes the accuracy given the hypervector size $\hvsize$ (and finds the optimal distance threshold for thresholding queries) for the data structure query encoded in the accuracy constraint.
%Because the accuracy analysis makes use of multiple analytical models that make different independence assumptions, this analysis additionally returns an \textit{independence constraint} that must hold for the analysis to be valid.
%Section~\ref{sec:mutual:independence} introduces the independence constraints.
Section~\ref{sec:model:intuition} presents the intuition of the analytical model, which is rigorously presented in Section~\ref{sec:analyticalmodel}.
Section~\ref{sec:thr:analysis} presents the accuracy analysis procedure for thresholding queries (\codein{thrAccAnalysis}), and Section~\ref{sec:wta:analysis} presents the accuracy analysis procedure for WTA queries (\codein{wtaAccAnalysis}).




\subsection{Accuracy Analysis for Thresholding Queries}

 
 
%\luke{So the notions like ``in-set'', ``not-in-set'' do not represent the subset case well; and ``$m$'', ``data structure size'' do not represent the type-III QDS well, where $\mu$ and $\sigma$ depend on the sizes of the ds multiplicant sets. Should we just say that this section is an illustrative example that uses type-I QDS?}
%\sara{definitely not.}



\subsubsection{\mycodeheading{Threshold Optimization}{getThreshold}}



\subsubsection{\mycodeheading{Accuracy Analysis Algorithm}{thrAccAnalysis}}\label{sec:thrAccAnalysis}
The accuracy analysis (\algname{thrAccAnalysis}) algorithm solves for the optimal threshold and lower accuracy bound for the query described in the accuracy constraint.
The algorithm pseudo code is shown in Figure~\ref{algo:get:accuracy}.
The \codein{thrAccAnalysis} function accepts as input a query and data structure, a hypervector size (\codein{n}), the minimum number of query elements contained within the data structure (\codein{k}), the hardware error model (\codein{hw}), an accuracy lower bound (\codein{reqAcc}) and a false positive rate/false negative rate upper bound (\codein{reqFp}, \codein{reqFn}). The accuracy analysis translates the hardware error model to a single bit flip error probability upper bound $p$ (Section~\ref{sec:inferbfp}) and then invokes the analytical model $\analyticalmodel(q,ds,k,n,hw)$ (Section~\ref{sec:analyticalmodel}) on the query and data structure HD expressions ($q$ and $ds$), the hypervector size ($n$), the hardware error probability $p$, and the number of query elements $k$ to derive the in-set and not-in-set distributions $\Phi_S,\Phi_{NS}$ and the mutual independence constraint $indepCstr$. 

 
 The algorithm then computes the optimal distance threshold $\threshold$ from distributions $\Phi_S,\Phi_{NS}$ that delivers false positive and false negative rate less than the false-positive/false negative upper bounds ($fp \leq reqFp$ and $fn \leq reqFn$) and maximizes the accuracy. If such a threshold cannot be found, the algorithm sets \codein{succ=\syn{false}}. Provided a threshold is successfully found ($succ=fp \leq reqFp \wedge fn \leq reqFn \wedge 1-\frac{fp + fn}2 \geq reqAcc$), the algorithm then returns the optimal threshold, the mutual independence constraint that must hold, and whether this parametrization satisfies the provided accuracy constraint ($\tuple{succ,indepCstr,\threshold}$).
 
\subsection{Accuracy Analysis for WTA Queries}\label{sec:wta:analysis}

The accuracy analysis procedure for WTA queries (\codein{wtaAccAnalysis}) also uses the analytical model $M$ to get the in-set and not-in-set distributions ($\Phi_S$ and $\Phi_{NS}$).
%The inputs of a WTA query are the number of winners $w$, a data structure vector $ds$ and a codebook of $m$ vectors, when it is known that $w$ vectors in $m$ are positives ($\distance{q}{ds}\sim \Phi_S$) and the other $m-w$ are negatives ($\distance{q}{ds}\sim \Phi_{NS}$).
The WTA queries assume that $w$ vectors in $m$ are positives ($\distance{q}{ds}\sim \Phi_S$) and the other $m-w$ are negatives ($\distance{q}{ds}\sim \Phi_{NS}$).
The WTA query simply returns the $w$ vectors that have the smallest distance to the data structure vector among the $m$ vectors in codebook.

\subsubsection{\mycodeheading{Accuracy Analysis Algorithm}{wtaAccAnalysis}}
Figure~\ref{algo:wta:accuracy} presents the pseudo code for WTA accuracy analysis.
Similarly as \codein{thrAccAnalysis}, it first gets $\Phi_S$ and $\Phi_{NS}$ from the analytical model (Section~\ref{sec:analyticalmodel}), then computes the expected accuracies $acc$ and $prob$ (Section~\ref{sec:wta:acc:compute}), for the two accuracy constraints respectively.
The accuracy $acc$ of the WTA query is the probability that the returned $w$ vectors are exactly the $w$ positives.
The first accuracy constraint requires $acc\ge x$.
The second accuracy constraint defines $prob$ as the probability that the $w$ positives are all among the top-$t$ in the codebook with the smallest distances to the data structure $ds$, and requires that $prob\ge x'$.
The analysis is successful iff the two constraints are both satisfied.
Finally the algorithm returns whether the analysis is successful, and the independent constraints.


==> old-texfiles/tech-models-backup.tex <==
\newcommand{\binomsum}[2]{S_{#1}^{#2}}

\section{\myheading{\tool{} Analytical Model ($\analyticalmodel$)}}\label{sec:analyticalmodel}

Given a query $q$, a data structure $ds$, a hardware error $hw$, a hypervector size $\hvsize$ and a query subset size $k$, \tool{} derives the symbolic mean and standard deviation expressions for the in-set and not-in-set distributions and the mutual independence constraint.
We start with the preliminaries and the definition of the independent constraints.

\subsection{Preliminaries}

\noindent\textbf{Code Tuples, Code Sets, and Code Tuple Sets.} A code $\code$ is a randomly generated hypervector that maps to a distinct atomic symbol (e.g., a letter), and a codebook $\codebook$ is a collection of codes.
A code set $\codes \subseteq \codebook$ is a vector that is the superposition (bundle, $\hdplus$) of a set of codes.
We denote $\code \in \codes$ if $\code$ is a code in the set, and $\codes=\set{\code_1,\code_2,\ldots,\code_m}$ if $\codes$ is a superposition of codes $\code_1 \hdplus{} \code_2 \hdplus{} \ldots \hdplus{} \code_m$.
%The $\size{\codes}$ function retrieves the maximum size of the code set $m$.
We denote a code tuple $\codetuple$ as a product ($\hdtimes$) of two or more codes, and create code tuples by binding codes, e.g., $\code \hdtimes \code' = \codetuple$. A code tuple set $\codetupleset$ is a set of code tuples.
The analysis works with codes, code tuples, code sets, and code tuple sets.

\noindent\textbf{Permutation Operator Elimination.}(\codein{eliminatePermute}) The permutation operators are eliminated by translating each permutation $\hdperm{\codebook}{i}$ to a distinct codebook $\codebook_{perm,i}$ where $\magnitude{\codebook} = \magnitude{\codebook_{perm,i}}$.
This transformation can be applied because each bit of a code $\code$ is independently randomly generated, and thus $\code$ and $\hdperm{\code}{k}$ can be viewed as two independent codes.
In other words, the dependency of $\code$ and $\hdperm{\code}{k}$ is negligible for computation. 


\subsection{Mutual Independence}\label{sec:mutual:independence}

The \tool{} analytical model assumes that both the data structure and query containing \textit{mutually independent} codes or tuples. In the analytical model, \tool{} identifies the mutual independence constraints that must hold. These mutual independence constraints are dynamically checked when constructing the data structure and query. The specific mutual independence constraint depends on the type of analytical procedure used to perform the analysis.

\subsubsection{Independent Set}\label{sec:independent:set:definition}
We define independent sets as a set of codes or tuples that are \emph{mutually independent}.
Formally, given any HD expression, it can be flattened into the superposition (set) of code tuples $\expr=\sum_{i=1}^lt_i$.
This $\expr$ is an independent set if and only if for any $t_i,1\le i\le l$, its vector cannot be inferred from the vectors of other tuples in the set.
For example, $\expr=(a\hdplus b)\hdtimes c\hdplus a\hdtimes b=a\hdtimes c\hdplus b\hdtimes c\hdplus a\hdtimes b$ is not an independent set, because $a\hdtimes b$ can be inferred from $a\hdtimes c$ and $b\hdtimes c$ by $a\hdtimes b=(a\hdtimes c)\hdtimes (b\hdtimes c)$.
Recalling a tuple in an independent tuple set is similar as recalling a code from a simple code set, because they follow the same distance distributions.

\subsubsection{Independent Product}\label{sec:independent:product:definition}
A product of sets $\expr=\hdtimes_{i=1}^ls_i$ is called an independent product if and only if the multiplicant sets are disjoint and the sum of all the multiplicant sets $\sum_{i=1}^ls_i$ is an independent set.
For example, $(a\hdplus b)\hdtimes (c\hdplus d)$ is an independent product because these two sets are disjoint and $a,b,c,d$ are mutually independent.
$(a\hdtimes b\hdplus a\hdtimes c)\hdtimes (b\hdtimes c\hdplus b\hdtimes d)$ is not an independent product because $a\hdtimes b, a\hdtimes c, b\hdtimes c,b\hdtimes d$ are not mutually independent, even though the two multiplicant sets are both independent sets.

Note that a product of sets can also be flattened into a set of tuples, and the flattened set is usually not independent, e.g., $(a\hdplus b)\hdtimes (c\hdplus d)=a\hdtimes c\hdplus a\hdtimes d\hdplus b\hdtimes c\hdplus b\hdtimes d$ is not an independent set because $(b\hdtimes c)\hdtimes (b\hdtimes d)\hdtimes (a\hdtimes d) = a\hdtimes c$.
%Therefore, product independence is a weaker constraint than set independence.

\subsection{Model Overview}

The \tool{} analytical model derives the in-set distribution parameters $\tuple{\mu_{S},\sigma_{S}}$, the not-in-set distribution parameters $\tuple{\mu_{NS}, \sigma_{NS}}$ for the provided query, and the mutual independence constraint $indepCstr$ that must hold for the analysis to be valid:

\vspace{3pt}
\begin{tabular}{rcl}
$\tuple{MeanDist_{S},MeanDist_{NS},indepCstr}$ & $=$ & $QDS(q,ds,n,k)$\\
$\tuple{\mu_{S},\sigma_{S}}$ & $=$ & $ToNormal(HwErr(hw, MeanDist_{S}))$\\
$\tuple{\mu_{NS},\sigma_{NS}}$ & $=$ & $ToNormal(HwErr(hw, MeanDist_{NS}))$\\
\end{tabular}
\vspace{3pt}

Sections~\ref{sec:qds}-\ref{sec:analysis:qds:3} describes how the in-set and not-in-set mean distances are derived from the query and data structure ($QDS$), Section~\ref{sec:hwerror} describes how hardware error is incorporated into the error-free mean distance ($HwErr$), and Section~\ref{sec:tonormal} derives the standard deviation from the mean of the same distance distribution ($ToNormal$).

\begin{table}
\centering
\footnotesize
\begin{tabular}{|c|c|c|}
\hline
\textbf{Formulation} & \textbf{reference} & \textbf{description}\\ \hline
WTA-$acc$, $w=1$ (\ref{eq:frady:wta:1}) & \cite{frady2018theory} &  WTA accuracy for exactly one winner\\
WTA-$acc$ (\ref{eq:wta:k}) & Section~\ref{sec:wta:acc:compute} & WTA accuracy for more than one winner\\
WTA-$prob$ (\ref{eq:wta:prob}) & Section~\ref{sec:wta:acc:compute} & probability of the $w$ positives being in top t.\\
QDS I (\ref{eq:set}) & \cite{kanerva1997fully} & single-element sum-of-product set membership\\
QDS II (\ref{eq:partialsubset}) & \cite{kleyko2016holographic} & subset sum-of-product set membership\\
QDS III (\ref{eq:nwayprod}) & Section~\ref{sec:analysis:qds:3} & single-element product-of-sum set memebership\\
Hardware Error (\ref{eq:distr}) & Section~\ref{sec:tonormal} & incorporation of hardware error\\
\hline
\end{tabular}
\caption{Summary of Theoretical Formulations}
\label{table:formulas}
\end{table}

We summarize the theoretical formulations (including formulations in the analytical model in this section, and the accuracy computation of WTA queries in Section~\ref{sec:wta:acc:compute}) in this paper in Table~\ref{table:formulas}.

\subsection{Query-Data Structure (QDS) Predicates}\label{sec:qds}

 We introduce the concept of a query-data structure (QDS) predicate, a unifying formalization that enables \tool{} to implement an analysis that both leverages theoretical results from previous literature~\cite{kleyko2021survey1,kleyko2022vector}, and the novel derivations (Section~\ref{sec:analysis:qds:3}). A query-data structure predicate is a set membership expression with the formulation $|q \cap ds|\ge k$ for which the symbolic in-set and not-in-set mean distances have been analytically derived. The \tool{} analysis supports three forms of QDS predicates (tuple $\codetuple$ and tuple set $\codetupleset$ can also be simply code $\code$ and code set $\codes$):

\vspace{3pt}
\begin{tabular}{ll}
    $|\set{\codetuple} \cap \codetupleset| \ge 1$ & \textbf{Type I, Single Element, Independent Tuple-Set} [Section~\ref{sec:analysis:qds:1}]\\
    $|\codetupleset \cap \codetupleset'| \ge k$ & \textbf{Type II, Subset, Independent Tuple-Set} [Section~\ref{sec:analysis:qds:2}]\\
    $|\set{\codetuple} \cap \codetupleset| \ge 1$ & \textbf{Type III, Single Element, Independent Product} [Section~\ref{sec:analysis:qds:3}]\\
\end{tabular}
\vspace{5pt}

Type I QDS predicates test if a code/tuple is in an independent code/tuple set, type II QDS predicates test if $k$ elements of a code/tuple set is a subset of an independent code/tuple set, and type III predicates test if a tuple is in an independent product.
Each QDS type is associated with an independence constraint on the data structures.
Type I QDS can be seen as a special case of type II QDS, but it is listed as a separate QDS as it is most frequently used.

Note that these 3 QDS predicates systematically cover all cases except for the subset query in the independent product.
Subsets of independent products may have dependent tuples, which are theoretically challenging~\cite{clarkson2023capacity}.
This kind of queries are rarely used in data structures~\cite{kleyko2021survey1,kleyko2022vector}.
We leave incorporating this kind of queries as future work.

\noindent\textbf{QDS Classification.} Given a query and data structure, \tool{} classifies the query into 3 supported QDS predicates by inspecting the data structure and the query expression form.
If the data structure is in the form of product of sums (bound tuple sets), then it must be a type III query and the query must be a tuple.
Otherwise, the data structure must be an independent code/tuple set, in the form of sum or products (bundle of code tuples).
Then if the query is a code set or code tuple set, it must be a Type II query.
If the query is a code or code tuple, then it must be a Type I query.

\noindent\textbf{Mutual Independence Constraints.}
Depending on the QDS Type, \tool{} returns a mutual independence constraint that must hold over the data structure for the corresponding analysis to be valid.
For sum-of-product formed data structure $\expr$, the independence constraints $indepCstr=iset($\expr$)$ requires that $\expr$ is an independent set (Section~\ref{sec:independent:set:definition}).
For product-of-sum formed data structure $\expr$, the independence constraint $indepCstr=iproduct($\expr$)$ requires that $\expr$ is an independent product (Section~\ref{sec:independent:product:definition}).

\subsection{Most Common Not-in-Set Distribution - Independent Vectors}\label{sec:analysis:independent}
We start with the simplest and the most commonly used not-in-set distribution - the distance distribution between two independent/unrelated vectors $\expr_1$ and $\expr_2$.
We denote the mean distance between two vectors $\expr_1$ and $\expr_2$ as $\meandist{\expr_1}{\expr_2}=\ev{\distance{\expr_1}{\expr_2}}$.
In the following analysis, we assume all the code sets and code tuple sets are of odd size.
The reason is that when bundling even number of vectors, the common practice is to add one more randomly generated vector as an operator to prevent the potential ties for majority~\cite{kleyko2021survey1}.

Because hamming distance is essentially the average distance across all vector dimensions, the mean distance between two vectors is then the probability of them to differ in any one dimension.
Since no correlation exists between two independent vectors, each dimension of one is equally likely (with probability $0.5$) to be 0/1 (same/different) from the perspective of the other.
The mean distance is therefore
{%\small
\begin{equation}\label{eq:independent}
    \meandist{\expr_1}{\expr_2} = \frac12, \forall\ \mathrm{independent}\ \expr_1,\expr_2
\end{equation}
}

\subsection{Type I (Single Element - Independent Set) Analytical Model}\label{sec:analysis:qds:1}

In this QDS type, the query is a code $\code$/tuple $\codetuple$ and the data structure is a code set $\codes$/tuple set $\codetupleset$.
Since the distance distributions in this QDS are the same for $|\set{\code}\cap\codes|\ge 1$ or $|\set{\codetuple}\cap\codetupleset|\ge 1$, we describe the $|\set{\code}\cap\codes|\ge 1$ case.
The query asks whether $\code\in \codes$.
Suppose $|\codes|=m$.
In the not-in-set case $|\set{\code}\cap \codes|<1$, i.e., $\code\notin \codes$, the mean distance is (\ref{eq:independent}) as the two vectors have no correlation.
The mean distance of the in-set case $\code\in \codes$ has been derived by Kanerva~\cite{kanerva1997fully}:
{%\small
\begin{equation}\label{eq:set}
    \meandist{\set{\code_1}}{\set{\code_1,\code_2,\ldots,\code_m}} = \frac{1}{2} - \frac{\binom{m-1}{\frac{m-1}{2}}}{2^m}
\end{equation}
}
For Type I QDS queries, equations (\ref{eq:set}) and (\ref{eq:independent}) are the in-set mean distance $MeanDist_S$, and not-in-set mean distance ($MeanDist_{NS}$) respectively. The independence constraint ($indepCstr$) for Type I queries requires all codes be mutually independent. ($iset{\set{\code_1,\code_2,\ldots,\code_m}}$)

\subsection{Type II (Subset - Independent Set) Analytical Model}\label{sec:analysis:qds:2}

QDS Type II queries are a generalization of Type I QDS.
In this QDS type, the query is a code set $\codes$/tuple set $\codetupleset$, and the data structure is a code set $\codes'$/tuple set $\codetupleset$.
Again, in this QDS type, the distance distributions are the same for $|\codes\cap \codes'|\ge k$ or $|\codetupleset\cap\codetupleset'|\ge k$, we describe the $|\codes\cap \codes'|\ge k$ case.
Assume $\codes'=\set{\code_1,\code_2,\ldots,\code_m}$, $\codes=\set{\code_1,\code_2,\ldots,\code_n,\code_1',\code_2',\ldots,\code_p'}$ has $l$ ($l\le m$) codes $\code_1,\code_2,\ldots,\code_l$ also in $\codes'$ and the $p$ other codes $\code_1',\code_2',\ldots,\code_p'$ not in $\codes'$.
The mean distance of $\codes$ and $\codes'$ in this case has been derived by Kleyko et al.~\cite{kleyko2016holographic}:
{\footnotesize
\begin{equation}\label{eq:partialsubset}
    \meandist{\set{\code_1,\code_2,\ldots,\code_l,\code_1',\code_2',\ldots,\code_p'}}{\set{\code_1,\code_2,\ldots,\code_m}} = 1-\frac1{2^{p+m-1}}\sum_{i=0}^{\min(\frac{l+p-1}{2},\frac{m-1}{2})}\binom{l}{i}\sum_{j=0}^{\frac{l+p-1}{2}-i}\binom{p}{j}\sum_{k=0}^{\frac{m-1}{2}-i}\binom{m-l}{k}
\end{equation}
}
For Type II QDS queries, equation (\ref{eq:partialsubset}) implements the in-set mean distance ($MeanDist_S$) when $p=k$, and the not-in-set mean distance ($MeanDist_{NS}$) when $p=k-1$. The Type II independence constraint ($indepCstr$) for Type II queries require both subset and set codes be mutually independent ($iset{\set{\code_1,\code_2,\ldots,\code_m}} \wedge iset{\set{\code_1,\code_2,\ldots,\code_l,\code_1',\code_2',\ldots,\code_p'}}$).


\subsection{Type III (Tuple-Set) Analytical Model }\label{sec:analysis:qds:3}
In this QDS type, the query vector is a code tuple $\codetuple$ and the data-structure vector is a product-of-sum formed code tuple set $\codetupleset=\hdtimes_{i=1}^l \codetupleset_i$, i.e., $\codetupleset$ is a binding of several code tuple sets.
We derive for this QDS type because binding code sets is a common operation used in constructing data structures, e.g., analogical database~\cite{kanerva2010we}, finite-state-automata~\cite{pashchenko2020search}.
Although $\codetupleset$ is also a tuple set (it can be flattened to sum-of-product form), this QDS type differs from type I in that the tuples in $\codetupleset$ have dependencies, while QDS type I assumes independence of tuples in the set.
For example, consider $\codetupleset=(\code_1\hdplus \code_2)\hdtimes (\code_3\hdplus \code_4)=\code_1\hdtimes \code_3+\code_1\hdtimes \code_4+\code_2\hdtimes \code_3+\code_2\hdtimes \code_4$.
The first tuple $\code_1\hdtimes \code_3$ is the binding of the other three.
The dependencies make the distance distributions different.

Since this analysis requires that $\codetupleset=\hdtimes_{i=1}^l \codetupleset_i$ is an independent product (Section~\ref{sec:independent:product:definition}), enabling us to view tuples in $\cup_{1\le i\le l}\codetupleset_i$ as independent codes, in the following analysis we assume $\codetupleset=\hdtimes_{i=1}^l \codes_i$, i.e. $\codetupleset$ is a product of code sets, and the results generalize to the $\codetupleset=\hdtimes_{i=1}^l \codetupleset_i$ case.
We first consider the simple case where $\codetupleset=\codes\hdtimes \codes'$ is the product of two code sets.
Assume $\codes=\set{\code_1,\code_2,\ldots,\code_l}$ is of size $l$ and $\codes'=\set{\code_1',\code_2',\ldots,\code_m'}$ is of size $m$.
The not-in-set case is $|\set{\codetuple}\cap \codetupleset|< 1$, i.e., $\codetuple\notin \codetupleset$, then the two independent vectors have mean distance (\ref{eq:independent}).
Otherwise, suppose $t=\code_1\hdtimes \code_1'$, we derive that
{\footnotesize
\begin{equation}\label{eq:twowayprod}
\begin{aligned}
    \meandist{\code_1\hdtimes \code_1'}{\set{\code_1,\code_2,\ldots,\code_l}\hdtimes \set{\code_1',\code_2',\ldots,\code_m'}} &= \frac{1}{2^{l+m-2}}\left[\left(\sum_{i=0}^{\frac{l-1}{2}}\binom{l-1}{i}\right)\left(\sum_{i=0}^{\frac{m-3}{2}}\binom{m-1}{i}\right)\right.\left.+\left(\sum_{i=0}^{\frac{l-3}{2}}\binom{l-1}{i}\right)\left(\sum_{i=0}^{\frac{m-1}{2}}\binom{m-1}{i}\right)\right]
\end{aligned}
\end{equation}
}
% {\small
% \begin{equation}\label{eq:twowayprod}
% \begin{aligned}
%     \meandist{\code_1\hdtimes \code_1'}{\set{\code_1,\code_2,\ldots,\code_l}\hdtimes \set{\code_1',\code_2',\ldots,\code_m'}} &= \frac{1}{2^{l+m-2}}\left[\binomsum{l-1}{\frac{l-1}2}\binomsum{m-1}{\frac{m-3}{2}}\right.\left.+\binomsum{l-1}{\frac{l-3}{2}}\binomsum{m-1}{\frac{m-1}{2}}\right]
% \end{aligned}
% \end{equation}
% }
The derivation is as follows.
Since binding is commutative, we have
{\small
\[
\begin{aligned}
    \distance{\code_1\hdtimes \code_1'}{\set{\code_1,\code_2,\ldots,\code_l}\hdtimes \set{\code_1',\code_2',\ldots,\code_m'}}&=\frac1{\hvsize}|(\code_1\hdtimes \code_1')\hdtimes (\set{\code_1,\code_2,\ldots,\code_l}\hdtimes \set{\code_1',\code_2',\ldots,\code_m'})|\\&=\frac1{\hvsize}|(\code_1\hdtimes \set{\code_1,\code_2,\ldots,\code_l})\hdtimes (\code_1'\hdtimes \set{\code_1',\code_2',\ldots,\code_m'})|\\&=\distance{\code_1\hdtimes \codes_1}{\code_1'\hdtimes \codes_1'}
    %&=\distance{\code_1\hdtimes \set{\code_1,\code_2,\ldots,\code_n}}{\code_1'\hdtimes \set{\code_1',\code_2',\ldots,\code_m'}}
\end{aligned}
\]
}
Therefore, for one dimension of $\codetuple$ and $\codetupleset$ to differ, either in the dimension $\code_1$ and $\codes$ are the same while $\code_1'$ and $\codes'$ differ, or the $\code_1'$ and $\codes'$ are the same while $\code_1$ and $\codes$ differ.
The probability of $\code_1$ and $\codes$ to be the same in a dimension is $\frac1{2^{l-1}}\sum_{i=0}^{\frac{l-1}{2}}\binom{l-1}{i}$ because it requires less than half (at most $\frac{l-1}2$) of $\code_2,\code_3,\ldots,\code_l$ to differ from $\code_1$ in the dimension, and the number of possible choices satisfying this is $\sum_{i=0}^{\frac{l-1}{2}}\binom{l-1}{i}$ and there are $2^{l-1}$ choices for $\code_2,\code_3,\ldots,\code_l$ in total.
For $\code_1$ and $\codes$ to be different in a dimension, there has to be at most $\frac{l-3}{2}$ of $\code_2,\code_3,\ldots,\code_n$ to be the same as $\code_1$ in the dimension, with probability $\frac1{2^{l-1}}\sum_{i=0}^{\frac{l-3}{2}}\binom{l-1}{i}$.
By symmetry, we also get the probability for $\code_1'$ and $\codes'$ to be the same or differ in one dimension.
Combining them together gives (\ref{eq:twowayprod}).

Note that the computation of (\ref{eq:twowayprod}) and (\ref{eq:partialsubset}) can be sped up by pre-computing the binomial coefficients and prefix sums of them with Pascal's triangle.

More generally, $\codetupleset$ can be the binding of $w,\forall w\ge 2$ sets.
Assume $\codetupleset = \hdtimes_{i=1}^w\codes_i$, and $\codes_i=\set{\code_{i1},\code_{i2},\ldots,\code_{il_i}}$ is a code set of size $l_i$.
In this general case, we have
{%\small
\begin{equation}\label{eq:nwayprod}
\begin{aligned}
    \meandist{\hdtimes_{i=1}^w\code_{i1}}{\hdtimes_{i=1}^w\set{\code_{i1},\code_{i2},\ldots,\code_{il_i}}} &= \frac{1}{2^{\sum_{i=1}^wl_i-w}}\sum_{\sum_{i=1}^we_i\mathrm{\ is\ odd}}\left[\prod_{j=1}^w\left(\sum_{k=0}^{\frac{l_i-1}{2}-e_i}\binom{l_i-1}{k}\right)\right]
\end{aligned}
\end{equation}
}

The derivation is similar as for (\ref{eq:twowayprod}).
By commutativity of binding, we have
{%\small
\[
\begin{aligned}
    \frac1{\hvsize}|(\hdtimes_{i=1}^w\code_{i1})\hdtimes (\hdtimes_{i=1}^w\set{\code_{i1},\code_{i2},\ldots,\code_{il_i}})|=\frac1{\hvsize}|\hdtimes_{i=1}^w(\code_{i1}\hdtimes \set{\code_{i1},\code_{i2},\ldots,\code_{il_i}})|\\
    %&=\distance{\code_1\hdtimes \set{\code_1,\code_2,\ldots,\code_n}}{\code_1'\hdtimes \set{\code_1',\code_2',\ldots,\code_m'}}
\end{aligned}
\]
}
Therefore, denoting $e_i$ as the value of one dimension of $\codes_{i1}\hdtimes \set{\code_{i1},\code_{i2},\ldots,\code_{il_i}})$ ($0$ or $1$), for $\codetuple\hdtimes \codetupleset$ to be $1$ in the dimension, odd number of $e_i$s should be $1$, i.e., $\sum_{i=1}^we_i$ is odd.
The probability for each $e_i$ to be $0$ or $1$ has been derived for (\ref{eq:twowayprod}).
Adding the probability of all the independent cases gives (\ref{eq:nwayprod}). Note that for large $w$, (\ref{eq:nwayprod}) is non-trivial to compute, as there are exponential number of cases where $\sum_{i=1}^we_i$ is odd.
However, common HDC computations do not involve binding of more than $2$ sets.
We leave the problem of computing (\ref{eq:nwayprod}) more efficiently to future work.

For Type III QDS queries, equation (\ref{eq:nwayprod}), or (\ref{eq:twowayprod}) when $w=2$ computes the in-set mean distance ($MeanDist_S$). Equation (\ref{eq:independent}) computes the not-in-set mean distance ($MeanDist_{NS}$). The mutual independence constraint ($indepCstr$) for this QDS query is $iproduct(\hdtimes_{i=1}^w\set{\code_{i1},\code_{i2},\ldots,\code_{il_i}})$.

\subsection{Hardware Error-Aware Mean Distance Model $HwErr(hw,MeanDist)$}\label{sec:hwerror}

HDC is a suitable computing paradigm for emerging hardware platforms because it is highly resilient against noises in them~\cite{halawani2021fused,imani2017exploring,imani2019sparsehd,karunaratne2020memory,poduval2021stochd}.
\tool{} incorporates the noise present in hardware, which works simultaneously for all the distance distributions above.
We consider the bit-flip error model, where the probability of each bit in hyper-vectors to flip is $p$.
We focus on its effect on distance calculation, as it is the only way HD computation retrieves information.
Bit flips change the mean distance between two vectors.
We model the change of mean distance after bit flips.
Denote $\bitflipmeandist{\expr_1}{\expr_2}$ as the mean distance of two vectors considering possible bit flips.
We have
{%\small
\begin{equation}\label{eq:bitflip}
    \bitflipmeandist{\expr_1}{\expr_2} = (p^2+(1-p)^2)\meandist{\expr_1}{\expr_2} + 2p(1-p)(1-\meandist{\expr_1}{\expr_2})
\end{equation}
}

The derivation is as follows.
$\meandist{\expr_1}{\expr_2}$ is the probability of two vectors to be the same in one dimension, and $\bitflipmeandist{\expr_1}{\expr_2}$ is the probability considering bit flips.
There are two cases where they are the same in one dimension with possible bit flips.
First, they can be the same before possible bit flips with probability $\meandist{\expr_1}{\expr_2}$, and then two vectors either both have a bit flip, or both have no bit flip in the dimension, with probability $p^2+(1-p)^2$.
Second, they differ before possible bit flips with probability $1-\meandist{\expr_1}{\expr_2}$, and a bit flip occurs only to one of the two vectors in this dimension, with probability $2p(1-p)$.

\noindent\textbf{Hardware errors increase the expected distance between vectors.} In all cases we consider, $\meandist{\expr_1}{\expr_2}\le \frac12$.
The maximum $\meandist{\expr_1}{\expr_2}$ is $\frac12$ when $\expr_1$ and $\expr_2$ are unrelated, as shown in (\ref{eq:independent}), and relatedness of vectors makes their mean distance smaller.
We show that possible bit flips increase the mean distances between vectors.
{%\small
\begin{equation}\label{eq:bitfliplargermean}
    \bitflipmeandist{\expr_1}{\expr_2}-\meandist{\expr_1}{\expr_2} = 2p(1-p)(1-2\meandist{\expr_1}{\expr_2}) \ge 0
\end{equation}
}
Larger mean distance means closer to distribution of unrelated vector, implying loss of relation information encoded in the hypervectors.
The implication is that hardware noise decreases the information resolution, which is intuitive.
We note that information loss increases with $p$ in a reasonable noise range, as in (\ref{eq:bitfliplargermean}) $2p(1-p)$ increases monotonically for $0<p<0.5$.
This enables us to use a upper bound of $p$ in our analysis and deliver a sound accuracy guarantee.

\subsubsection{Bit-Flip Probability}\label{sec:inferbfp}
We derive the bit flip error probability from the hardware specification $hw$.
As a standard practice, raw bit flip error rate is commonly used to characterize hardware noises.~\cite{le2021radar, grossi2019resistive, li2016hyperdimensional}
Given the hypervector operators and memory locations $op \in Op =$ \{\codein{bind}, \codein{bundle}, \codein{codebook}, \codein{item\hyphen{}mem}, \codein{query}\} 
from the hardware specification, we denote the error of an operator as $\hwerror{op}$. We can compute the $p$ as follows:

{%\small
\[
\begin{aligned}
p &=& 1-[\product_{op \in Op} (1-\hwerror{op})]
%(1-\hwerror{bundle})(1-\hwerror{bind})\times (1-\hwerror{distance})\times (1-\hwerror{permute})\ &&\times (1-\hwerror{codebook}) \times (1-\hwerror{item\hyphen{}mem}) \times (1-\hwerror{query})
\end{aligned}
\]}

$p$ captures the probability of at least one bit flip happens in certain operator or memory location.
Note that $p$ is a probability upper bound of a bit flip occurs in query or data structure during distance calculations, and using $p$ delivers sound accuracy analysis as the information loss increases with $p$ in a reasonable range $0<p<0.5$ (shown in (\ref{eq:bitfliplargermean})).

\subsection{Correspondance between Mean Distance and Distance Distributions ($ToNormal$)}\label{sec:tonormal}

Given a mean distance $\bitflipmeandist{\expr_1}{\expr_2}$ considering bit flips and hypervector size $\hvsize$, we can derive the standard deviation and mean to get the corresponding normal distribution $N(\mu,\sigma)$. Denote $x$ as the value of one dimension in $\expr_1 \hdtimes \expr_2$.
Note that $\distance{\expr_1}{\expr_2}=\frac1{\hvsize}|\expr_1 \hdtimes \expr_2|$.
Since $x$ is either $0$ or $1$, the following holds:
{\small
\[
\ev{x^2}=\ev{x}=\bitflipmeandist{\expr_1}{\expr_2},
Var[x]=\ev{x^2}-E^2[x]=\bitflipmeandist{\expr_1}{\expr_2}(1-\bitflipmeandist{\expr_1}{\expr_2})
\]
}
Since all $\hvsize$ dimensions in $\expr_1 \hdtimes \expr_2$ are independent and symmetric, we have
{\small
\[
    Var[\distance{\expr_1}{\expr_2}]=\frac1{\hvsize} Var[x]=\frac1{\hvsize} \bitflipmeandist{\expr_1}{\expr_2}(1-\bitflipmeandist{\expr_1}{\expr_2})
\]
}
To sum up, the distance distribution is determined by the mean distance and hypervector size $\hvsize$.
{\small
\begin{equation}\label{eq:distr}
    \distance{\expr_1}{\expr_2}\sim N\left(\bitflipmeandist{\expr_1}{\expr_2}, \sqrt{\frac1{\hvsize} \bitflipmeandist{\expr_1}{\expr_2}(1-\bitflipmeandist{\expr_1}{\expr_2}})\right)
\end{equation}
}

==> old-texfiles/tech-outline.tex <==
\section{\tool{} Overview}

%Figure: Optimizer (section listed), WTA analysis, threshold analysis, analytical model (section attached), dynamic analysis.

% static optimizer produces a concrete, optimized program from specs. 

% runtime takes optimized program, parameterizes HD computation, performs necessary dynamic checks + threshold selection for analysis to hold.

\section{\tool{} Optimizer}

\noindent\textbf{Algorithm.}

\section{Accuracy Analysis}

%analysis works with an analytical model, here's intuitively what it looks like. See section XXX for derviation.

\subsection{Analytical Model Intuition}

% interface of analytical model (inputs and outputs)

% intuition behind what model computes.


\subsection{Threshold-based Accuracy Analysis [XXX]}

\subsection{WTA-Based Accuracy Analysis [XXX]}


\section{Analytical Model Derivation [XXX]}

\begin{table}
\begin{tabular}
model component&reference&description\\
QDS I & \cite{XXX} & set-subset membership\\
Hardware Error & novel & XXX\\
\end{tabular}
\caption{Analytical model summary}
\end{table}
% formalization here
\noindent\textbf{Formalization.}

% overview here
\noindent\textbf{Overview.} The novel components of this model include XXX.

\subsection{Mutual Independence Constraints}


\subsection{QDS Predicates}


\subsubsection{Type I: XXX}


\subsubsection{Type II: XXX}


\subsubsection{Type III: XXX}

\subsection{Hardware Error Extension}



\section{\tool{} Runtime}

\section{Discussion}

==> result_old.tex <==
\section{Evaluation}\label{sec:results}

We evaluate \tool{} on the analysis-amenable data structures presented in Section~\ref{sec:datastructures} and supplementary materials.
% Appendix~\ref{sec:datastructure:appendix}.
% Appendix~\ref{sec:benchmarks:detailed}
Refer to the supplementary materials for a detailed description of the benchmark applications. For each data structure benchmark, we select 5 specifications in which Heim optimized hypervector size $\hvsize$ is around 10,000. For each specification we randomly empirically evaluate accuracy over 100 random instantiations of the data structure with 20 queries each. We generate data structures with not too small sizes to sufficiently test baselines' capabilities.
% Appendix~\ref{sec:benchmarks:detailed}
%Refer to the supplementary materials for the benchmark program implementations.
Each randomly instantiated data structure query is executed for 10 simulation trials, where each simulation trial generates new random codebook vectors.

\noindent\textbf{Benchmarks.} We use the following benchmarks.
% (Appendix~\ref{sec:datastructure:set})
\begin{itemize}[leftmargin=*,label=$\tinybullet$]
\item\textbf{\codein{set}} We choose 100, 200, 300, 400, 500 as the maximum set sizes $MAX$ in 5 specifications, and for each $MAX$ construct 100 random sets data structures, each containing $[\frac{MAX}{2},MAX]$ codes. We generate 20 random codes as queries. Around 50\% queries are in the set and 50\% are not in the set. The query tests if a code is in the set. 

%(Appendix~\ref{sec:datastructure:database})
\item\textbf{\codein{db-match}} We choose 5 specifications with (max length of records $MRLEN$, length of the match $MLEN$) being (10, 2), (20, 4), (30, 6), (40, 8), (50, 10) respectively. For each specification we first generate a match consisting of $MLEN$ key-value pairs, and then we construct 100 random databases consisting of $[50,100]$ records, each record has length of $[\frac{MRLEN}{2},MRLEN]$. Around 50\% records match, and the other 50\% match a random number of values. We query the match in the database with all records.

%(Appendix~\ref{sec:datastructure:database})
\item\textbf{\codein{db-wta-analogy}} We choose 5 specifications with (max length of records $MRLEN$, max number of records $MR$) being (4, 100), (8, 200), (12, 300), (16, 400), (20, 500) respectively. We construct 100 random databases for each specification with $[\frac{MR}{2}, MR]$ records, each having a length of $[\frac{MRLEN}{2}, MRLEN]$. Different records have different values for the same keys. We then construct 20 analogy queries for each database by randomly selecting two records with common keys. For this benchmark, all the baselines use WTA query approach.

\item\textbf{\codein{db-thr-analogy}} We choose 5 specifications with ($MRLEN$, $MR$) being (2, 50), (4, 100), (6, 150), (8, 200), (10, 250) respectively. The data structure and query construction follow the same procedure as benchmark \codein{db-wta-analogy}. For this benchmark, all the baselines use thresholding query approach. Note that the data structure sizes are smaller compared to benchmark \codein{db-wta-analogy} because thresholding performs worse than wta for this type of queries.

\item\textbf{\codein{knowledge-graph}} (Section~\ref{sec:datastructure:knowledgegraph}) We choose 100, 200, 300, 400, 500 as the maximum specified degrees $MD$. We construct 100 random instantiations of a ($MD+10$)-vertex, 2-relation knowledge graphs with 10 nodes having $[\frac{4MD}{5},MD]$ edges to the other $MD$ nodes. For each graph, we randomly generate 20 edge queries and test whether they match with the 10 nodes with outgoing edges.

%(Appendix~\ref{sec:datastructure:nfa})
\item\textbf{\codein{nfa}} We evaluate our nondeterministic finite automatas (NFA) on substring search task~\cite{pashchenko2020search}.
We choose 6, 8, 10, 12, 14 as the base string length.
For eeach base string length, we randomly generate 100 base strings, and for each base string we generate 20 random query strings, in which half are random substrings of the base string, and the other half randomly partially match the base string.
All the strings are generated with the alphabet of lower-case English letters.
%
%We construct 800-1000 nondeterministic finite automatas (NFA) that recognizes strings of length 8-20. The query operation constructs 2 random query strings with a length of 1-10 and counts the number that are correctly recognized by the NFA.
\end{itemize}

\noindent\textbf{Accuracy Metric.} We use the following accuracy metrics and statistics.
\begin{itemize}
    \item \codein{accuracy} - Given \codein{P} in-set query invocations and \codein{N} not-in-set query invocations that produce \codein{TP} true positive and \codein{TN} true negative results, the accuracy of each benchmark is defined as the average of the true positive and true negative rates ($\frac 1 2 (\frac{TP}{P} + \frac{TN}{N})$). We generate an approximately equal number of positive and negative queries for each benchmark.
    We evaluate on a balanced strategy to view false positive rate and false negative rate as equally important because the real distributions of positive and negative queries are dependent on the target applications. Our specification language supports unbalanced false positive and false negative rates, so unbalanced query distributions can also be handled. 
    \item \codein{med}, \codein{iqr}, \codein{min}, \codein{max}, and \codein{std} the median, inter-quartile-range, minimum, maximum and standard deviation of accuracies on 100 random instantiations of data structures for each benchmark of a specific size.
    \item \codein{rat} the percentage ratio of the 100 random data structures that have no less than the specified (99\%) accuracy.
\end{itemize}


\noindent\textbf{Baselines.} We evaluate the following baselines on the benchmarks to evaluate \tool{} against the traditional static approach and dynamic thresholding, and to investigate \tool{}'s performance on emerging, error-prone hardware technologies:

\begin{itemize}[leftmargin=*,label=\tinybullet]
%\item\textbf{\codein{\tool{}-nom} and \codein{\tool{}-thr}} We statically optimize the thresholds and hypervector size for each benchmark with \tool{}, and perform error free hardware simulation on the optimized benchmark. For \codein{\tool{}-thr}, we fix the hypervector size to 10,000 and statically optimize the thresholds for each benchmark with \tool{}.
\item\textbf{\codein{\tool{}-nom}} We statically optimize the thresholds and hypervector size for each benchmark with \tool{} to get 99\% accuracy, and perform error free hardware simulation on the optimized benchmark.

%\item\textbf{\codein{bl-thr}} We set the hypervector size to 10,000 bits and empirically tune the distance threshold to get the best accuracy metric using the algorithm discussed in Section~\ref{sec:example:dynamic:tuning}. We try up to 1000 thresholds, and execute 1 simulation trial per threshold. This baseline is compared against the \codein{\tool{}-thr} executions to evaluate the efficacy of \tool{}'s threshold optimizer. 
\item\textbf{\codein{bl-static}} We set the hypervector size to 10,000 bits and empirically tune a distance threshold to get the best accuracy metric using the algorithm discussed in Section~\ref{sec:example:dynamic:tuning}. We tune on 10 random data structures with 20 queries each on 1 random codebook.

\item\textbf{\codein{bl-dt}} We binary search the hypervector size. For each size empirically tune a threshold as in \codein{bl-static}. The binary search finds the smallest hypervector size that reaches 99\% accuracy with the tuned threshold. The binary search upper bound is set to $100000$. If hypervector size $100000$ with a tuned threshold cannot achieve the target 99\% accuracy, the algorithm uses $100000$.

\item\textbf{\codein{\tool{}-2bpc} and \codein{\tool{}-3bpc}} We statically optimize the thresholds and hypervector size for each benchmark with \tool{} against a resistive memory hardware error model to get 99\% accuracy, and simulate bit-per-cell (BPC) and 3BPC ReRAM item memory storage by injecting bit-flip errors into item memory hypervectors. The 2BPC and 3BPC ReRAM raw bit error rates are \codein{0.0215} and \codein{0.1273} respectively. All ReRAM error measurements were collected by characterizing a fabricated ReRAM storage array without error correction.~\cite{wei2023dala}
The ReRAM array has 65536 cells, and is fabricated with 130nm logic CMOS process in the BEOL.~\cite{hsieh2019high,le2021radar}

\end{itemize}

\subsection{Resource Efficiency of \tool{}}\label{sec:results:resource}

\begin{figure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/Set_Theory_Cells_BitFlip.pdf}
\caption{\codein{set}}
\label{fig:storage:set}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/match_Theory_Cells_BitFlip.pdf}
\caption{\codein{db-match}}
\label{fig:storage:match}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/KG_Theory_Cells_BitFlip.pdf}
\caption{\codein{knowledge-graph}}
\label{fig:storage:kg}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/NFA_Theory_Cells_BitFlip.pdf}
\caption{\codein{nfa}}
\label{fig:storage:nfa}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/thr_a_Theory_Cells_BitFlip.pdf}
\caption{\codein{db-thr-analogy}}
\label{fig:storage:thr:analogy}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/wta_a_Theory_Cells_BitFlip.pdf}
\caption{\codein{db-wta-analogy}}
\label{fig:storage:wta:analogy}
\end{subfigure}
% \begin{subfigure}[b]{0.74\textwidth}
% \small
% \centering
% \setlength{\tabcolsep}{1.5pt}
% \begin{tabular}{|c|cc|cc|cc|cc|cc|}
% \hline
%  & \multicolumn{2}{c|}{\textbf{set}}  & \multicolumn{2}{c|}{\textbf{db-match}} & \multicolumn{2}{c|}{\textbf{db-analogy}} & \multicolumn{2}{c|}{\textbf{graph}} & \multicolumn{2}{c|}{\textbf{nfa}}\\
%  \textbf{benchmark}&\textit{mean}&\textit{std}& \textit{mean}&\textit{std}& \textit{mean}&\textit{std}& \textit{mean}&\textit{std}& \textit{mean}&\textit{std}\\
% \hline
% \codein{\tool{}-nom} & 99.04 & 0.12 & 99.10 & 0.29 & 99.18 &0.52 & 99.75 & 0.34 & 99.50 & 0.85 \\
% \codein{\tool{}-2bpc} & 99.00 & 0.07 & 98.96 & 0.18 & 99.03 & 0.46 & 99.75 & 0.33 & 99.25 & 1.41 \\
% \codein{\tool{}-3bpc} & 99.00 & 0.05 & 99.05 & 0.20 & 99.00 & 0.32 & 99.75 & 0.34 & 99.31 & 1.19 \\
% \hline
% %\codein{\tool{}-nom} & (0.9904,0.0012) & (0.9910,0.0029) & (0.9918,0.0052) & (0.9975,0.0034) & (0.9944,0.0140) \\
% %\codein{\tool{}-2bpc} & (0.9900,0.0007) & (0.9896,0.0018) & (0.9903,0.0046) & (0.9975,0.0033) & (0.9950,0.0122) \\
% %\codein{\tool{}-3bpc} & (0.9900,0.0005) & (0.9905,0.0020) & (0.9900,0.0032) & (0.9975,0.0034) & (0.9381,0.0480) \\
% \end{tabular}
% \caption{Measured \% accuracy (\codein{accuracy $\times$ 100\%}), target accuracy is \codein{99.0}\%}
% \label{table:empirical:accuracy}
% \end{subfigure}


\caption{Memory cells required to store each hypervector with \codein{99\%} accuracy. The \swatch{black} is unoptimized hypervector size (10,000 bits, 1-bit-per-cell), \swatch{skyblue} is \codein{\tool{}-nom}, \swatch{tangerine} is 
 \codein{\tool{}-2bpc}, \swatch{pixelgreen} is \codein{\tool{}-3bpc}. \codein{db-match} records use 20 fields, \codein{db-thr-analogy} databases have 100 records, \codein{db-wta-analogy} databases have 300 records.}
 \label{fig:storage}
\end{figure}

\input{big_exp_table}


\begin{figure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/Set_runtime.pdf}
\caption{\codein{set}}
\label{fig:runtime:set}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/Match_runtime.pdf}
\caption{\codein{db-match}}
\label{fig:runtime:match}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/KG_runtime.pdf}
\caption{\codein{knowledge-graph}}
\label{fig:runtime:kg}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/NFA_runtime.pdf}
\caption{\codein{nfa}}
\label{fig:runtime:nfa}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/thr_analogy_runtime.pdf}
\caption{\codein{db-thr-analogy}}
\label{fig:runtime:thr:analogy}
\end{subfigure}
\begin{subfigure}[b]{0.30\textwidth}
\includegraphics[width=\linewidth]{figures/wta_analogy_runtime.pdf}
\caption{\codein{db-wta-analogy}}
\label{fig:runtime:wta:analogy}
\end{subfigure}


\caption{Measured runtimes for tuning the hypervector size and threholds. The \swatch{skyblue} is \codein{\tool{}-nom}, \swatch{tangerine} is 
 \codein{bl-dt}.}
 \label{fig:runtime}
\end{figure}
% \begin{figure}
% \small
% \centering
% \setlength{\tabcolsep}{1.5pt}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% & \textbf{set-500} & \textbf{kg-500} & \textbf{wta-a-20-500} & \textbf{thr-a-10-250} & \textbf{match-50-10} & \textbf{nfa-14}\\ \hline
% \textbf{\codein{\tool{}-nom} (ms)} & 121 & 122 & 1588 & 126 & 307 & 83\\ \hline
% \textbf{\codein{bl-dt} (hhmmss)} & 00:03:21 & 00:56:32 & 22:43:19 & 01:34:04 & 12:48:24 & 04:12:34\\ \hline

% \end{tabular}
% \caption{Measured tuning runtime for \codein{\tool{}-nom} and \codein{bl-dt}, on the largest benchmarks}
% \label{table:runtime}
% \end{figure}

We optimize the five benchmark applications to minimize resource usage while delivering a target accuracy of \codein{0.99} or \codein{99\%}. Figure~\ref{fig:storage} presents the number of memory cells required to store each hypervector as a function of data structure and query complexity.

\tool{} produces hypervectors that require 76-8400 binary memory cells, reducing the hypervector size by a factor of 1.19x-131.58x compared with \codein{bl-static}. \tool{} produces 94-10064 bit hypervectors that use 47-5032 memory cells for 2 BPC ReRAM, netting an additional 1.614x-1.677x cell reduction over conventional binary memory. We observe though the overall hypervector size increases for 2 BPC memory, the 2x improvement in data density for this memory technology subsumes this size increase. \tool{} produces 270-27361 bit hypervectors that use 90-9121 memory cells for 3 BPC ReRAM. Though 3 BPC ReRAM is denser than 2 BPC ReRAM, it does not net density improvements for the benchmark HD computations. By leveraging \tool{}, we can perform principled analysis of the promise of different device hardware technologies for HD comptutations.



\subsection{Comparison to Static Approach and Dynamic Thresholding}\label{sec:results:compare}

% \begin{figure}
% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\linewidth]{figures/Set_ACC_Compare.pdf}
% \caption{\codein{set}}
% \label{fig:threshold:set}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\linewidth]{figures/Database_Analogy_Corr.pdf}
% \caption{\codein{db-analogy}}
% \label{fig:threshold:dbanalogy}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\linewidth]{figures/Database_Matching_ACCR.pdf}
% \caption{\codein{db-match}}
% \label{fig:threshold:dbmatch}
% \end{subfigure}
% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\linewidth]{figures/Knowledge_Graph_Accuracy.pdf}
% \caption{\codein{knowledge graph}$\dagger$}
% \label{fig:threshold:graph}
% \end{subfigure}

% \begin{subfigure}[b]{0.24\textwidth}
% \includegraphics[width=\linewidth]{figures/String_Matching_accr.pdf}
% \caption{\codein{nfa}$\dagger$}
% \label{fig:threshold:nfa}
% \end{subfigure}
% \begin{subfigure}[b]{0.73\textwidth}
% \centering
% \small
% \begin{tabular}{|c|ccccc|}
% \hline
%  \textbf{benchmark} & \textbf{set}  & \textbf{db-match} & \textbf{db-analogy} & \textbf{graph} & \textbf{nfa}\\
% \hline
% \codein{\tool{}-nom} & 0.0871 & 0.1891 & 0.0378 & 9.3440 & 0.0361 \\
% \codein{bl-thr} & 15851 & 5049.9 & 1065.7 & 1171.1 & 3464.9 \\
% \hline
% \end{tabular}
% \caption{Parameter optimization times (ms) for the largest problem size in each benchmark.}
% \label{table:runtimes}
% \end{subfigure}

% \caption{Average reported accuracies (0.0-1.0) benchmark executions vs. increasing query complexity. \swatch{tangerine} for \codein{bl-thr} accuracy,  \swatch{skyblue} for \codein{\tool{}-thr} accuracy, \swatch{brickred} dotted line is \tool{}-derived theoretical accuracy. $\dagger$theoretical accuracy is lower bound..}
% \label{fig:threshold}
% \end{figure}

We compare \codein{\tool{}-nom} against \codein{bl-static} and \codein{bl-dt}.
\tool{} minimizes the hypervector size while achieving the 99\% accuracy with the derived optimal threshold.
Figure~\ref{table:empirical:accuracy} compares the derived dimension and accuracy measures of HD computations on the 6 benchmarks.
Note that \codein{bl-dt} uses $\hvsize=100000$ for some benchmarks because it cannot find a tuned threshold achieving the target 99\% accuracy even with the maximum size $100000$.
We make the following observations.
\begin{itemize}
    \item \textbf{\tool{} achieves higher accuracy, and the median reaches the desired 99\% more reliably.} \tool{} achieves 99.2\%-100.0\% median accuracy, with 100.0\% in 19 benchmarks, and the median is no less than 99\% in all benchmarks. \codein{bl-static} achieves 54.5\%-100.0\% median accuracy, and the median is no less than 99\% in only 16 benchmarks, which are mainly small benchmarks. \codein{bl-dt} achieves 60.0\%-100.0\% median accuracy, and the median is no less than 99\% in only 4 benchmarks.
    \item \textbf{\tool{}'s hypervector sizes and thresholds generalize better and more consistently achieves the specified 99\% accuracy in random data structures. \codein{bl-dt}'s tuned sizes and thresholds generalize poorly to random data structures with similar complexity.} \tool{} achieves 80.0\%-100.0\% ratio, and the ratio is no less than 90\% in 26 benchmarks. \codein{bl-static} achieves 0.0\%-100.0\% ratio, and the ratio is no less than 90\% in 11 benchmarks, which are mainly small benchmarks. \codein{bl-dt} achieves 0.0\%-99.0\% ratio, and the ratio is no less than 90\% in only 3 benchmarks.
    \item \textbf{\tool{} is more robust and achieves higher accuracy in worst cases.} \tool{} achieves 97.0\%-99.0\% minimum accuracy, \codein{bl-static} achieves 44.0\%-100.0\% minimum accuracy, and \codein{bl-dt} achieves 52.0\%-98.5\% minimum accuracy.
    \item \textbf{\tool{}'s accuracies in random data structures have less variations.} \tool{}'s accuracy has 0.0-0.5 inter-quartile-range (iqr) and 0.1-0.6 standard deviation (std), \codein{bl-static}'s accuracy has 0.0-7.5 iqr and 0.0-5.2 std, and \codein{bl-dt}'s accuracy has 0.0-5.0 iqr and 0.2-3.6 std. \tool{}'s iqr are no greater than \codein{bl-dt}'s in all but one (\textbf{kg-200}, due to sample variation) benchmarks, and \tool{}'s std is no greater than \codein{bl-dt}'s in all benchmarks. \codein{bl-static}'s iqr and std are lower only in small benchmarks.
    \item \textbf{\tool{} usually uses larger hypervector sizes than \codein{bl-dt}, as \tool{} statically optimizes for the worst cases, while \codein{bl-dt} dynamically tunes for random cases. \tool{} and \codein{bl-dt} are able to adjust the hypervector sizes based on benchmark sizes to minimize resource usage.} \luke{Sara looks at this} \tool{}'s hypervector sizes are 857-41186, and \codein{bl-dt}'s hypervector sizes are 489-100000. \tool{}'s hypervector sizes are 1.01x-2.46x larger than \codein{bl-dt}'s in 21 benchmarks, and 4.52x-27.82x smaller in 9 benchmarks. \tool{}'s and \codein{bl-dt}'s hypervector sizes are smaller in small benchmarks and larger in large benchmarks than \codein{bl-static}'s.
\end{itemize}
% We observe that \tool{} can derive dimensions and thresholds in various data structure sizes, which stably achieve the target 99\% accuracy across random data structures, as its iqr and std are nearly always smaller than \codein{bl-dt}.
% Besides, \tool{} has much higher ratio (\codein{rat}) of the sampled data structures that gets a $\ge 99\%$ accuracy measured on $20$ queries and $10$ codebooks, with \codein{rat} in most benchmarks $>90\%$, while \codein{bl-dt}'s is in most benchmarks $<50\%$.
% In comparison, the static approach cannot adapt to larger data structure sizes and have accuracy much less than 99\% for larger data structures.
% The dynamically tuned dimensions and thresholds on a few random data structures do not generalize as well to other random data structures, as the achieved accuracy is in many cases lower than 99\%, and using only \emph{one} threshold performs poorly in \codein{match} and \codein{nfa} benchmarks.


\noindent\textbf{Optimization Time.} Figure~\ref{fig:runtime} compares the optimization times for \tool{} against the \codein{bl-dt} baseline. \textbf{\tool{}'s parameter optimization is 3-5 orders of magnitude faster, and is more scalable than \codein{bl-dt}}. 
\tool{} completes its analysis in 85-3210 millisconds, while \codein{bl-dt} takes anywhere from around 40 seconds to over 22.72 hours to complete its analysis.
\codein{bl-dt} uses 303.0x-100167.4x more time than \tool{}, with a geometric mean of 11214.4x.
\tool{} attains better performance than dynamical tuning because dynamic thresholding approaches requires Monte Carlo simulation to derive a threshold.
Dynamic tuning scales poorly with the number of simulation trials and parameters to tune.
In contrast, \tool{}'s static analysis procedure is model-based and can compute the optimal threshold and hypervector size with constant time that is independent of the data structure size.

==> results-scratch.tex <==
\begin{itemize}[leftmargin=*,label=\tinybullet]
\item \textbf{\codein{EMBEDDED}}: This hardware platform emulates a typical embedded microcontroller device. It has 2 cores and 2 threads, 1GHz CPU frequency and a 3-level cache. The level 1 cache has 32KB data cache and 64KB instruction cache (both are 8-way associative) for each core. The level 2 cache is 2MB, 16-way associative. The level 3 cache is 16MB, 16-way associative.
~\cite{imani2017exploring} 

\item \textbf{\codein{MULTICORE}}: This hardware platform emulates a typical multi-core computer processor. It has 10 cores and 20 threads, 2.8GHz CPU frequency and a 3-level cache. The level 1 cache has 32KB data cache and 32KB instruction cache (both are 8-way associative) for each core. The level 2 cache is 256KB, 4-way associative. The level 3 cache is 20MB, 16-way associative.

\item \textbf{\codein{CAM}}: This hardware platform emulates an embedded microcontroller with content addressable memory (CAM) for faster distance calculation. The query encoding runs on an embedded microcontroller with the same parameters as \codein{EMBEDDED}., and extrapolate with a linear model for latency numbers not reported in the paper.
\end{itemize}


==> tech-scratch.tex <==


 \begin{figure}[t]
 \small
\begin{minipage}{\linewidth}
%\small
\begin{algorithmic}[1]
\Procedure{wtaAccAnalysis}{hw,n,\lit{wta-query}(q,ds,k,w,m,x,t,x')}
%\State \textbf{float} p = \lit{getBitFlipProb}(hw)
\State $\tuple{indepCstr,\Phi_M,\Phi_{NM}}$ = $\analyticalmodel(q,ds,k,n,hw)$
\State $\tuple{acc,prob}$ = \lit{computeWTAAccuracies}($\Phi_M,\Phi_{NM}$,w,m,t)
\State $success$ = $acc\ge x\wedge prob\ge x'$
\State \textbf{return} $\tuple{success,indepCstr}$
\EndProcedure
\end{algorithmic}
\caption{\tool{} \algname{wtaAccAnalysis} algorithms \luke{There should be a \lit{binsearch} procedure as it is invoked by the optimizer}}
\label{algo:wta:accuracy}
\end{minipage}
\end{figure}

- area under overlapping region is error probability, left of threshold 

\noindent\textbf{Accuracy of Winner-Take-All Queries.} \todo{Sara make a pass} For winner-take-all (WTA) queries, the \textit{accuracy} is determined by computing the probability that all the match queries (whose distances to the data structures are samples from the match distribution) have smaller distances than all the non-match queries (whose distances to the data structures are samples from the non-match distribution), i.e., the positives are the ones with the smallest distances.
Accuracy = probability blue points on the left of the red points. No notion of one blue point being more of a match than the other.
probability none of the top k points are drawn from the red distribution -- all topk points drawn from blue.
wta-query(e,e',k,w,m,x,t,x')



k = # of matched elements in subset

WTA returns top w matches, given an item memory of m elements. Given a true set of w matches $\omega$, the hard accuracy constraint enforces that the top w matches come from $\omega$ with probability $x$, and the soft accuracy constraint enforces that $\omega$ is contained within the top $t$ matches. The former ensures we only return correct results with high probability, and the latter ensures that if we retrieve a larger set of matches, the correct matches will be contained within that set. Winner take all queries will always draw from a set of matches.

The accuracy constraint enforces the hard requirement that the top w matches come from the match distribution with probability x, and the softer requirement that the top w points are contained in the top t matches.

probability that all of the top w points come from match distribution = accuracy probability (we want it to be $\ge x$). We won't return a match that is not contained in data structuure.

probability that all w points from match distribution are in top t elements, where w <= t  <= m (we want it to be $\ge x'$), can set slack on match.

\noindent\textbf{Expected Accuracy.} 


\todo{need to redo figure to talk about it.}


(\codein{k=1}) query \codein{q} made against each row in the data structure \codein{ds} should correctly classify each row in the data structure's item memory with a probability $probAcc$, 

\todo{figure mods: 10 items in item memory, single query.}
\todo{w instead of k for top matches in WTA}

Given a query $q$, a data structure $ds$, a hardware bit error probability $p$, a hypervector size $\hvsize$ and a query subset size $k$, \tool{} derives the symbolic mean and standard deviation expressions for the match and not-match distributions.
Figure~\ref{fig:distr} visualizes the match and not-match analytical models. Given a data structure query $|q \cap ds|\ge k$ with hypervector size $\hvsize$ and a hardware error probability $p$, \tool{} constructs symbolic match ($|q \cap ds|\ge k$) and not-match ($|q \cap ds|< k$) analytical distance distributions, which are modeled as normal distributions with a symbolic mean and standard deviation. The match and not-match probability distributions capture the distribution of distances between the query and data structure hypervectors $\distance{q}{ds}$ when the query matches the data structure ($|q \cap ds|\ge k$) and and the query does not match the data structure ($|q \cap ds|< k$) respectively.  The query and data structure parameters $ds$, $q$, and $k$ are computed from the \texttt{thr-query} and \texttt{wta-query} statements in the \tool{} specification, the hardware bit error probability is computed from the \tool{} error model, and the hypervector size $\hvsize$ is selected by the optimizer.


Intuitively, the match distribution captures the probability that at least $k$ elements in the query are contained within the data structure, and the not-match distribution captures the probability that less than $k$ in the query are contained within the data structure. Both match and not-match distances follow probability distributions rather than resolve to a concrete value. The query-data structure distance is non-deterministic because the codebook $\codebook$ is randomly generated, and the hardware non-deterministically introduces error into the stored hypervectors, and into the hypervector computations. The overlapping area between the match and not-match distributions is the probability that a query is erroneously misclassified -- because the distance distributions overlap, there is ambiguity on whether the query matches data structure or not. The degree of separation between the two distributions depend on the parametrization of the HD computation.


These statically derived thresholds and sizes are used to optimize HD computations and individual HD distance calculations on the fly. Section~\ref{sec:datastructures} presents a library of analysis-amenable data structures that uses \tool{} optimize query thresholds and hypervector sizes while still delivering accuracy guarantees. In the event \tool{} cannot find a hypervector size that satisfies all of the accuracy requirements, it reports that the parameter optimization problem is unsatisfiable. This \algname{optimize} algorithm uses the threshold query and winner-take-all query accuracy analyses presented in sections Section~\ref{sec:accuracyanalysis}, and makes use of the following helper functions:

\begin{itemize}[leftmargin=*,label={$\tinybullet{}$}]
\item\textbf{\algname{getConstraints}(accSpec)}: Returns the accuracy and hypervector dimension constraints found in the \tool{} accuracy specification (\codein{accSpec}). The query and data structure HD expressions in the accuracy constraint are expanded (through variable substitution) to implement expressions over products, sums, and permutations of basis vectors.
\item\textbf{\algname{binSearch}(min,max,accFun)}: Performs a binary search over integer values contained within $[min,max]$ to find the smallest value of $n$ that causes $accFun(n)$ to return true. Returns $max+1$ if no value is found.
\end{itemize}


The optimization algorithm derives the optimal hypervector size (and optimal threshold for thresholding queries) for each data structure query with an accuracy requirement. The hypervector size is found by performing a binary search over hypervector sizes in \codein{[0,maxN]} (Line 4-5, 13-14), and the optimal distance threshold is derived by analyzing the distance distributions in conjunction with the required accuracy bounds. \tool{} uses query accuracy analysis procedures to determine wither each query constraint can be satisfied, given a candidate hypervector size. The threshold-based query accuracy analysis procedure (\codein{thrAccAnalysis}) returns the optimal threshold for a given threshold-based query that satisfies the provided accuracy requirements ($reqFp$, $reqFn$, $reqAcc$), if one exists. The winner-take-all accuracy analysis procedure determines whether a given winner-take-all query's accuracy requirements ($x$, $t$, $x'$) are satisfied for a given hypervector size. These analyses are used to filter out hypervector sizes that do not meet the desired accuracy requirements imposed by each query, and are used to compute query-specific distance thresholds.


\noindent\textbf{Final Result.} After all of the accuracy constraints have been processed, the algorithm finds the largest hypervector dimension \codein{optDim} required by the set of constraints. Finally, the algorithm returns the optimal hypervector dimension and the set of query-specific hypervector dimensions and thresholds. 

\begin{figure}[t]
\begin{minipage}{\linewidth}
\footnotesize
\begin{algorithmic}[1]

\Procedure{optimizeThreshold}{thrCstrs,hw,maxN}
\State dims, params = \set{}, \set{}
\For{queryCstr = \lit{thr-query}(q,ds,k,reqAcc,reqFp,reqFn) $\in$ thrCstrs}
   \State{\textbf{fn} accFun = $\lambda{}$n.\lit{thrAccAnalysis}(hw,n,queryCstr).\lit{success}}
    \State{\textbf{int} n = \lit{binSearch}(0,maxN,accFun)}
    \State{$\tuple{\texttt{success,indepCstr,\threshold}}$ = \lit{thrAccAnalysis}(hw,n,queryCstr)}
    \State{dims = dims $\cup$ \{n\}}
    \State{params = params $\cup\set{\tuple{\texttt{indepCstr,\threshold,n}}}$}
\EndFor
\State \textbf{return} $\tuple{\texttt{dims,params}}$
\EndProcedure

\Procedure{optimizeWTA}{wtaCstrs,hw,maxN}
\State dims, params = \set{}, \set{}
\For{queryCstr = \lit{wta-query}(q,ds,k,w,m,x,t,x') $\in$ wtaCstrs}
   \State{\textbf{fn} accFun = $\lambda{}$n.\lit{wtaAccAnalysis}(hw,n,queryCstr).\lit{success}}
    \State{\textbf{int} n = \lit{binSearch}(0,maxN,accFun)}
    \State{$\tuple{\texttt{success,indepCstr}}$ = \lit{wtaAccAnalysis}(hw,n,queryCstr)}
    \State{dims = dims $\cup$ \{n\}}
    \State{params = params $\cup\set{\tuple{\texttt{indepCstr,n}}}$}
\EndFor
\State \textbf{return} $\tuple{\texttt{dims,params}}$
\EndProcedure

\Procedure{optimize}{hw,accSpec,maxN}
\State \textbf{set} wtaCstrs, thrCstrs = \lit{getConstraints}(accSpec)
 \State wtaDims, wtaParams = optimizeWTA(wtaCstrs,hw,maxN)
 \State thrDims, thrParams = optimizeThreshold(thrCstrs,hw,maxN)
\State{optDim = \lit{max}(wtaDims, thrDims)}
\If{optDim > maxN}
\State \texttt{\lit{error}("violation of dimensional constraints")}
\EndIf
\State \textbf{return} $\tuple{\texttt{optDim,wtaParams,thrParams}}$
\EndProcedure
\end{algorithmic}
\caption{\tool{} optimization algorithm. \codein{wtaAccAnalysis} and \codein{thrAccAnalysis} are presented in Section~\ref{sec:wta:analysis} and Section~\ref{sec:thr:analysis} respectively.}
\label{algo:opt}
\end{minipage}
\end{figure}

The static analysis workflow is as follows. The end users first specify the targeted hardware platform with a hardware error model, then provide description and specification of the data structure (maximum sizes) and queries (maximum sizes, desired accuracy).
The analysis-amenable data structures generate \tool{} specification accordingly for \tool{} static optimizer.
With the \tool{} specification, the \tool{} static optimizer employs an optimization algorithm (Section~\ref{sec:optimizer}).
The optimization algorithm binary searches to find the hypervector size that satisfies the accuracy constraints and minimizes resource usage.
The optimization algorithm uses an accuracy analysis procedure (Section~\ref{sec:accuracy:analysis}) that analyzes the accuracy and optimal query thresholds for the queries given the hypervector size.
The mathematical core of the accuracy analysis procedure is an analytical model (Section~\ref{sec:analyticalmodel}).
The analytical model takes as input the HD expressions of data structures and queries, some query parameters, and the hardware error model, outputs the distance distributions for the accuracy analysis procedure to complete its analysis.
Meanwhile, the analytical model identifies the mutual independence constraints required for the analysis to be valid.
Finally the \tool{} static optimizer returns the mutual independence constraints, the optimal hypervector sizes that meet the accuracy constraints and minimize the resource usage, and associated thresholds for executing thresholding queries.
% \tool{} runtime component then checks if the provided data structures are valid for analysis.
% Finally, concrete hypervectors are generated and queries are executed with parameters provided by the \tool{} static optimizer.
Note that end users are not confined by the analysis-amenable data structures we provide, and can use \tool{} static optimizer and runtime components to optimize their own HD computing, by describing the data structures used and the queries with \tool{} specification language.

The core of the static system is the \tool{} static optimizer.
% With the optimizer we build several analysis-amenable data structures (Section~\ref{sec:datastructures}) that provide clean APIs for users.
% They generate \tool{} specification and get the optimal hypervector sizes and thresholds statically with \tool{} optimizer, check the validity of data structures with \tool{} runtime component, generate the hypervectors, and execute the queries with them.
We next focus on the \tool{} static optimizer, which consists of an optimizer algorithm, accuracy analysis procedure, and an analytical model.
We present the optimizer algorithm in Section~\ref{sec:optimizer}.
The accuracy analysis is presented in Section~\ref{sec:accuracy:analysis} and the analytical model is presented in Section~\ref{sec:analyticalmodel}.



The details of the analysis-amenable data structures and the runtime system are in Section~\ref{sec:datastructures} and Section~\ref{sec:runtime} respectively.


==> tech-systemoverview.tex <==
\newpage
\section{\tool{} Optimizer Overview}\label{sec:overview}

\begin{figure}
\includegraphics[width=0.99\linewidth]{figures/HeimOverview.pdf}
\caption{Overview of \tool{} static analysis. The optimizer algorithm is elaborated in section~\ref{sec:optimizer}, accuracy analysis in section~\ref{sec:accuracy:analysis}, and analytical model in section~\ref{sec:analyticalmodel}.}
\label{fig:overview}
\end{figure}

% \begin{Verbatim}
% def optimizeWTA(..):
%     for wta-accuracy(...) \in wtaCstrs:
%         fn wtaAcc = \lambda n.wtaAccAnalysis(...).success
%         int n = binSearch(0,maxN,wtaAcc)
%         <succ, indepCstr> = wtaAccAnalysis(...)
%         OptDims = OptDims \cup {n}
%         QParams = QParams \cup {<...>}
%     return <max(OptDims), QParams)

% def optimizeThr(...):
%     ...
    
% def optimize(hw,accSpec,maxN):
%     set wtaCstrs, thrCstrs = getConstraints(accSpec)
%     nWTA, WTAParams = optimizeWTA(..)
%     nThr, ThrParams = optimizeThreshold(..)
%     assert(nOpt > maxN)
%     return <max(nWTA,nTHR), WTAParams, ThrParams>


% thrAccAnalysis // section 6.2
% wtaAccAnalysis // section 6.3


% \end{Verbatim}

The \tool{} optimizer finds the optimal hypervector length and query distance thresholds for an HD computation formalized in the \tool{} specification language.  \tool{} accepts as input a \tool{} specification, which formally describes the operation of a data structure, and a hardware error model for the target hardware platform and returns the optimal hypervector size and a collection of optimal, query-specific hypervector size and distance threshold values. 

\noindent\textbf{Optimal Sizes and Thresholds.}\tool{} returns the smallest hypervector size that satisfies all query accuracy requirements on the target hardware platform, and a set of query-specific distance thresholds and hypervector sizes for each query in the \tool{} specification. The threshold-based queries use the query-specific distance thresholds to identify if the query data is/is not in the data structure hypervector, and the query-specific sizes can be used to soundly perform the partial computation of specific queries. For queries involving sets of elements, \tool{} produces an optimal parametrization for each set size in the query hypervector.

\noindent\textbf{System Overview.} At the heart of \tool{} is the accuracy analysis (Figure~\ref{fig:overview:analysis}).

Given a hypervector size, a hardware error model, and a query accuracy constraint, \tool{} finds the d

Figure~\ref{fig:overview} presents an overview  \tool{} static optimizer. The static optimizer consists of three components:

\begin{itemize}[leftmargin=*]

\item{}\textbf{Analytical Model (Section~\ref{sec:analyticalmodel}).} We develop analytical models of the distance distribution between query and data structure hypervectors -- these models account for the effect of hardware error on hypervector distance. To build a complete analytical model that covers all queries supported by the \tool{} specification language and reasons about hardware error, we derive new theoretical results as part of this work. 


\item{}\textbf{Accuracy Analysis (Section~\ref{sec:accuracy:analysis}).} Given a query and hypervector size, the accuracy analysis derives the success probability of the given query on the target hardware and returns the derived success probability and optimal set of query parameters. The accuracy analysis works with analytical models of the hypervector distance distributions to compute the success probability.

\item{}\textbf{Optimization Algorithm (Section~\ref{sec:optimizer}).} The \tool{} optimization algorithm searches over candidate hypervector lengths to find the smallest hypervector length that satisfies the accuracy constraints. 
\end{itemize}

\noindent\textit{Mutual Independence Constraints.} Because a subset of analytical derivations requires certain independence properties to be true for the analysis, the analytical model also provides a set of independence constraints that must be enforced over the data structure. These constraints are enforced dynamically, at runtime, by \tool{}'s runtime system (Section~\ref{sec:runtime})

